$\epsilon$-Subgradient Algorithms for Bilevel Convex Optimization

This paper introduces and studies the convergence properties of a new class of explicit $\epsilon$-subgradient methods for the task of minimizing a convex function over the set of minimizers of another convex minimization problem. The general algorithm specializes to some important cases, such as first-order methods applied to a varying objective function, which have computationally cheap iterations. We present numerical experimentation regarding certain applications where the theoretical framework encompasses efficient algorithmic techniques, enabling the use of the resulting methods to solve very large practical problems arising in tomographic image reconstruction.

==> algo_.tex <==
\section{Theoretical Analysis}\label{sec:theoretical}

% \subsection{Classical Results}
% 
% Taking $f_1 = c$ in~\eqref{eq:bilevel} we recover the traditional
% single-level convex optimization problem. Assuming also, for the 
% sake of exposition, that we have $\epsilon_k = 0$ throughout 
% iterations~\eqref{eq:cabot}, then
% \begin{equation}
%    \vect x_{k + 1} = \vect x_k - \lambda_k\vect t_{k + 1},
% \end{equation}
% where $\vect t_{k + 1} \in \partial f_0( \vect x_{k + 1} )$. Now,
% let us define, for a closed convex $C$, the projection operator:
% \begin{equation*}
%    \mathcal P_C( \vect x ) := \argmin_{\vect y \in C}\| \vect x - \vect y \|.
% \end{equation*}
% 

\subsection{Stepsize Considerations}

Recall from the theory of $\epsilon$-subgradient
methods~\cite{col93} for the one level case (that is,
problem~\eqref{eq:bilevel} with $f_1 \equiv 0$)
that weak convergence of iterations~\eqref{eq:tobac} to a
solution, under mild extra assumptions of subgradient boundedness,
can be ensured with slowly diminishing stepsizes satisfying:
\begin{equation*}\label{eq:lambdaassump}\tag{A${}_\lambda$}
   \sum_{k = 0}^\infty\lambda_k = \infty\quad\text{and}\quad
   \lambda_k \to 0^+\text.
\end{equation*}
The non-summability hypothesis seems necessary. Vanishing stepsizes, however, may have the negative effect of slowing down asymptotic convergence of the algorithm. Therefore, owing to its computationally cheap iteration, methods like~\eqref{eq:tobac} are usually thought to be most competitive when the problem size is very large, or when highly accurate solutions are not required. However, in some important particular (with smooth interior objective function $f_0$) cases supported by the theory developed here, the stepsize $\lambda_k$ does not necessarily have to vanish and in such applications we obtain reasonably fast algorithms. Both cases are evaluated in the experimental work we present.

For the classical (one level) convex optimization problem,
proximal methods~\cite{roc76} require $\lambda_k \geq
\underline\lambda$ for some $\underline\lambda > 0$. For the
bilevel case, the same stepsize requirement, with an extra 
upper boundedness assumption, i.e.,
\begin{equation*}\label{eq:cabotlambda}\tag{C${}_\lambda$}
    0 < \underline\lambda \leq \lambda_k \leq \overline\lambda,
\end{equation*}
would ensure convergence of~\eqref{eq:cabot}
to the optimizer of~\eqref{eq:bilevel}.
For such results to hold~\cite{cab05}, the extra assumption of a
\emph{slow control}:
\begin{equation*}\label{eq:caboteta}\tag{C${}_\eta$}
    \sum_{k=0}^\infty \eta_k = \infty\quad\text{and}\quad \eta_k \to 0^+,
\end{equation*}
was made in order to ensure that the influence of $f_1$ throughout the iterations was strong enough while still becoming arbitrarily small. The alternative form below is more appropriate to us this time, as it will generalize immediately to our algorithms:
\begin{equation*}\label{eq:slowcontrol}\tag{A${}_\eta$}
   \sum_{k = 0}^\infty \lambda_k\eta_k = \infty
   \quad\text{and}\quad \eta_k \to 0^+\text.
\end{equation*}
Notice that if~\eqref{eq:cabotlambda} holds, then~\eqref{eq:slowcontrol} is equivalent  to~\eqref{eq:caboteta}. However, because the net  contribution to each iteration from $\partial f_1( \vect x_k )$ in algorithm~\eqref{eq:tobac} is actually $O( \lambda_k\eta_k )$, \eqref{eq:slowcontrol} generalizes to the case $\lambda_k \to 0^+$, while~\eqref{eq:caboteta} does not.

\subsection{Formal Algorithm Description}

The stepping stone of our analysis will be an abstract
three-step algorithm given as follows:
\begin{equation}\label{eq:algo}
   \begin{split}
      \vect x_{k + 1 / 3} &{}:= \mathcal{O}_{f_0}( \lambda_k, \vect x_k )\text;\\
      \vect x_{k + 2 / 3} &{}:= \mathcal{O}_{f_1}( \mu_k, \vect x_{k + 1 / 3} )\text;\\
      \vect x_{k + 1} &{}:= \mathcal{P}_{X_0}( \vect x_{k + 2 / 3} )\text,
   \end{split}
\end{equation}
where the operators $\mathcal{O}_{f_i}$ for $i \in \{ 0, 1 \}$ have very specific conceptual roles and must satisfy certain corresponding properties, which we will discuss right next. Sequences $\{ \lambda_k \}$ and $\{ \mu_k \}$ are stepsize sequences. The first one plays, in this abstract setting, the same role it plays in iterative scheme~\eqref{eq:tobac}, while sequence $\{ \mu_k \}$ will be identified with $\{ \lambda_k\eta_k \}$ when we later show that, under mild conditions, explicit method~\eqref{eq:tobac} is a special case of the abstract algorithm~\eqref{eq:algo}. Therefore, application of $\mu_k=\lambda_k\eta_k$ in~\eqref{eq:slowcontrol} leads immediately to
\begin{equation*}\label{eq:muassump}\tag{A${}_\mu$}
   \sum_{k = 0}^\infty\mu_k = \infty\quad\text{and}\quad
   \frac{\mu_k}{\lambda_k} \to 0^+\text.
\end{equation*}

Let us then describe the properties required for the \emph{optimality operators} $\mathcal O_{f_i}$. The imposed characteristics are easy to meet, as we later illustrate.

\begin{property}\label{prop:propopt1}
   There is $\beta > 0$ such that for any $\lambda \geq 0$ and for all $\vect x_{k + i / 3}$, $\vect y \in \mathbb R^n$, and $i \in \{ 0, 1 \}$:
   \begin{multline}\label{eq:propopt1}
      \| \mathcal O_{f_i}( \lambda, \vect x_{k + i / 3} ) - \vect y \|^2 \leq \| \vect x_{k + i / 3} - \vect y \|^2 - \beta\lambda\bigl( f_i\bigl( \mathcal O_{f_i}( \lambda, \vect x_{k + i / 3} ) \bigr) - f_i( \vect y ) \bigr)\\
      {} + \lambda\rho_i( \lambda, k )\text,
   \end{multline}
   where $\rho_i( \lambda, k )$ represents an error term, with properties to be describe later.
\end{property}

% \begin{property}\label{prop:propopterrvan}
%    For $i \in \{ 0, 1 \}$, and with $\rho_i$ as given by
%    the above property, there holds
%    \begin{equation*}
%       \lim_{\lambda \to 0^+}\rho_i( \lambda ) = 0\text;
%    \end{equation*}
% \end{property}
% 
\begin{property}\label{prop:propoptbound}
   There exists $\gamma > 0$ such that
   \begin{equation*}
      \| \vect x - \mathcal{O}_{f_i}( \lambda, \vect x )
      \|_2 \leq \lambda\gamma\text.
   \end{equation*}
\end{property}

Property~\ref{prop:propopt1} guarantees that, going from some fixed $\vect x$, the operator $\mathcal O_{f_i}$ will approach a point $\vect y$ with improved $f_i$ value if only the result of the operation does not have a better $f_i$ value than $\vect y$ and the stepsize $\lambda$ is small enough.
% Given Property~\ref{prop:propopterrvan}, this means that with
% small enough stepsizes the algorithm proceeds towards desired
% directions after application of the optimality operator, unless
% the iterate already has an objective value smaller than the
% constrained optimal.
Property~\ref{prop:propoptbound} is no
more than a boundedness assumption on the operators.

These can be derived from somewhat standard hypothesis for $\epsilon$-subgradient
algorithms (see, e.g., \cite{col93}) and, as such, a
plethora of concrete realizations of such operators is
possible, the most obvious being $\epsilon$-subgradient steps:
\begin{equation}
   \mathcal S_f( \lambda, \vect x ) := \vect x -
   \lambda\tilde\nabla_{\epsilon} f( \vect x
   )\text,
\end{equation}
where $\tilde\nabla_\epsilon f( \vect x ) \in
\partial_\epsilon f( \vect x )$. In this case we have:
\begin{equation}\label{eq:subgradstepineq}
   \|\mathcal S_f( \lambda, \vect x ) - \vect y\|_2^2 \leq
   \| \vect x - \vect y \|_2^2 - 2\lambda\bigl( f( \vect x )
   - f( \vect y ) \bigr) + \lambda\bigl( \lambda \|
   \tilde\nabla_{\epsilon}f( \vect x ) \|_2^2
   + 2\epsilon \bigr)\text.
\end{equation}
Furthermore, convexity leads to
\begin{equation}
   f\bigl( \vect x - \lambda \tilde\nabla_{\epsilon} f( \vect x ) \bigr) \geq f( \vect x ) - \lambda \tilde\nabla f( \vect x )^T\tilde\nabla_{\epsilon} f( \vect x ),
\end{equation}
where $\tilde\nabla f( \vect x ) \in \partial f( \vect x )$. This with~\eqref{eq:subgradstepineq} gives
\begin{multline}\label{eq:subgradstepineqB}
   \|\mathcal S_f( \lambda, \vect x ) - \vect y\|_2^2 \leq
   \| \vect x - \vect y \|_2^2 - 2\lambda\bigl( f( \mathcal S_f( \lambda, \vect x ) )
   - f( \vect y ) \bigr) \\
   {} + \lambda\bigl( \lambda \| \tilde\nabla_{\epsilon}f( \vect x ) \|_2^2 + 2\epsilon + 2\lambda \tilde\nabla f( \vect x )^T\tilde\nabla_{\epsilon} f( \vect x ) \bigr)\text,
\end{multline}
so that we can satisfy Properties~\ref{prop:propopt1}~and~\ref{prop:propoptbound} if we further assume $\epsilon$-subgradient boundedness (and consequently subgradient boundedness).

A straightforward generalization of the argument leading from~\eqref{eq:subgradstepineq} to~\eqref{eq:subgradstepineqB}, omitted for brevity, results in the following statement, which will be useful later:
\begin{proposition}\label{prop:oneIsOther}
   Assume an operator $\mathcal O_f : \mathbb R \times \mathbb R^n \to \mathbb R^n$ satisfies, for $\lambda > 0$
   \begin{equation}
      \|\mathcal O_f( \lambda, \vect x ) - \vect y\|_2^2 \leq \| \vect x - \vect y \|_2^2 - 2\lambda\bigl( f( \vect x ) - f( \vect y ) \bigr) + \lambda\varrho( \lambda )\text,
   \end{equation}
   where $\varrho( \lambda )$ is an error term, and
   \begin{equation}
      \|\mathcal O_f( \lambda, \vect x ) - \vect x\| \leq \lambda\gamma,
   \end{equation}
   for some $\gamma > 0$. Then, we have:
   \begin{equation}
      \|\mathcal O_f( \lambda, \vect x ) - \vect y\|_2^2 \leq \| \vect x - \vect y \|_2^2 - 2\lambda\bigl( f( O_f( \lambda, \vect x ) ) - f( \vect y ) \bigr) + \lambda\bigl( \varrho( \lambda ) + 2 \lambda\gamma\|\tilde\nabla f( \vect x )\| \bigr)\text,
   \end{equation}
   where $\tilde\nabla f( \vect x ) \in \partial f( \vect x )$.
\end{proposition}

Our analysis will focus on algorithms more general than~\eqref{eq:tobac}, allowing simple constraint sets $X_0$ to be handled. In order to simplify exposition, we use projections onto $X_0$ to ensure feasibility, but all we need is an operator that outputs a feasible point and also obeys the following:
\begin{property}\label{prop:propfac}
   For all $\vect x \in \mathbb R^n$ and $\vect y \in X_0$, we have
   \begin{equation}\label{eq:propfacforte1}
      \| \proj_{X_0}( \vect x ) - \vect y \| \leq \| \vect x - \vect y \|\text.
   \end{equation}
\end{property}

% Notice that orthogonal projection steps onto $X_0$ immediately satisfy this condition with $\eta_k \equiv 0$, so that projected $\epsilon$-subgradient algorithms will
% fit our theoretical framework.

% Moreover, we will show how
% to, under mild assumptions, build practical iterative operators 
% $\mathcal F_{X_0}$ such that, given some fixed $\varepsilon > 0$, 
% the above holds for convex sets $X_0$ of the form
% \begin{equation*}
%    X_0 = \{ \vect x\in \mathbb R^n : g_i( \vect x ) \leq 0,
%    i = 1, \dots, r \},
% \end{equation*}
% with $g_i : \mathbb R^n \to \mathbb R$ convex functions.%, in
%subsection~\ref{subsec:feaop}.

\subsection{Convergence Results}

We introduce some simplifying notations:
\begin{itemize}
   \item $f_i^*$ is the optimal value of $f_i$ over $X_i$;
   \item $X_{i + 1} := \{ \vect x \in X_i : f_i( \vect x )
   = f_i^*\}$.
\end{itemize}

Our first statement concerns the difference between successive iterations. That the magnitude of this difference vanishes under diverse circunstances will be of fundamental importance in later convergence proofs. In the following we have a straightforward result, useful for diminishing stepsizes. Potentially non-vanishing $\{\lambda_k\}$ will be also considered, in which case, instead of the result below, we provide other means of proving that the distance between successive iterates vanishes.

\begin{proposition}
   Suppose $\mathcal P_{X_0}$ satisfies \eqref{eq:propfacforte1}, and $\mathcal O_{f_0}$ and $\mathcal O_{f_1}$ satisfy Property~\ref{prop:propoptbound}. Then
   \begin{equation}\label{eq:iterdiffboundFinal}
         \| \vect x_{k + 1} - \vect x_{k} \| \leq 2d_{X_0}( \vect x_{k} ) + 3( \lambda_k + \mu_k )\gamma.
   \end{equation}
\end{proposition}
\begin{proof}
   First let us use the triangular inequality and Property~\ref{prop:propoptbound} of $\mathcal O_{f_0}$ and $\mathcal O_{f_1}$ in order to get:
   \begin{equation}\label{eq:iterdiffboundInter}
      \begin{split}
         \| \vect x_{k + 1} - \vect x_{k} \| & {} = \| \vect x_{k + 1} - \vect x_{k + 2/3} + \vect x_{k + 2/3} - \vect x_{k + 1/3} + \vect x_{k + 1/3} - \vect x_{k} \| \\
         & {} = \| \vect x_{k + 1} - \vect x_{k + 2/3} \| + \| \vect x_{k + 2/3} - \vect x_{k + 1/3} \| + \| \vect x_{k + 1/3} - \vect x_{k} \| \\
         & {} \leq \| \vect x_{k + 1} - \vect x_{k + 2/3} \| + ( \lambda_k + \mu_k )\gamma.
      \end{split}
   \end{equation}
   Using now the triangular inequality followed by inequality~\eqref{eq:propfacforte1} and finally by Property~\ref{prop:propoptbound} of $\mathcal O_{f_0}$ and $\mathcal O_{f_1}$, we have, for every $\vect z \in X_0$:
   \begin{equation}\label{eq:feabound}
      \begin{split}
         \| \vect x_{k + 1} - \vect x_{k + 2/3} \| & {} = \| \vect x_{k + 1} - \vect z + \vect z - \vect x_{k + 2/3} \| \\
         & {} \leq \| \vect x_{k + 1} - \vect z \| + \| \vect z - \vect x_{k + 2/3} \| \\
         & {} \leq 2\| \vect z - \vect x_{k + 2/3} \| \\
         & {} = 2\| \vect z - \vect x_{k} + \vect x_{k} - \vect x_{k + 1/3} + \vect x_{k + 1/3} - \vect x_{k + 2/3} \| \\
         & {} \leq 2\| \vect z - \vect x_{k} \| + 2( \lambda_k + \mu_k )\gamma.
      \end{split}
   \end{equation}
   Then, using~\eqref{eq:feabound} with $\vect z = \proj_{X_0}( \vect x_k )$ in~\eqref{eq:iterdiffboundInter} we get:
   \begin{equation}\label{eq:iterdiffboundFinal}
         \| \vect x_{k + 1} - \vect x_{k} \| \leq 2d_{X_0}( \vect x_{k} ) + 3( \lambda_k + \mu_k )\gamma.
   \end{equation}
\end{proof}

Our first result shows weak convergence (that is, in objective function value) of the iterates to the set of minimizers of $f_0$ over $X_0$. We next prove weak convergence to the set of minimizers of $f_1$ over $X_1$. Both of these preliminary results contain certain technical and some strong hypothesis. We subsequently weaken and clarify such \emph{ad hoc} requirements in order to obtain our main results.

\begin{proposition}\label{prop:CX}
   Assume that $X_1 \neq \emptyset$, $X_1$ is bounded (or $\{ \vect x_{k} \}$ is bounded) $\sum_{i = 0}^\infty \lambda_k = \infty$, $\mathcal O_{f_0}$ and $\mathcal O_{f_1}$ satisfy Property~\ref{prop:propopt1}, $f_1( \vect x_{k + 2 / 3} ) \geq \underline f > -\infty$, $\| \vect x_{k + 1 / 3} - \vect x_{k + 2 / 3} \| \to 0$, $\| \vect x_{k} - \vect x_{k + 1 / 3} \| \to 0$, $\rho_0( \lambda_k, k ) \to 0$, $\rho_1( \mu_k, k ) \leq \overline\rho_1 < \infty$, $\mu_k / \lambda_k \to 0$. Suppose also that there exists $M$ such that $\forall \vect z \in \{ \vect x_{k} \}$ there is $\vect v \in \partial f_0( \vect z )$ for which $\| \vect v \| < M$, then we have
   \begin{equation*}
      \lim_{k\to\infty}d_{X_1}( \vect x_k ) = 0\text.
   \end{equation*}
\end{proposition}

\begin{proof}
   We first notice that because the non-expansiveness of the projection and of  Property~\ref{prop:propopt1} of $\mathcal O_{f_0}$ and $\mathcal O_{f_1}$, there holds, for $\vect y \in X_1$:
   \begin{equation}\label{eq:lemmCXaux1}
      \begin{split}
         \| \vect x_{k + 1} - \vect y \|^2 & {} \leq \| \vect x_{k + 2 / 3} - \vect y \|^2 \\
         &{}\leq \| \vect x_{k + 1 / 3} - \vect y \|^2 - \beta\mu_k\bigl( f_1( \vect x_{k + 2 / 3} ) - f_1( \vect y ) \bigr) + \mu_k\rho_1( \mu_k, k ) \\
         &{} \leq \| \vect x_{k} - \vect y \|^2 - \beta\lambda_k\bigl( f_0( \vect x_{k + 1 / 3} ) - f_0^* \bigr) + \lambda_k\rho_0( \lambda_k, k ) \\
         & \qquad\qquad\qquad\qquad {} - \beta\mu_k\bigl( f_1( \vect x_{k + 2 / 3} ) - f_1( \vect y ) \bigr) + \mu_k\rho_1( \mu_k, k )\text.
      \end{split}
   \end{equation}
   Denote $N = f_1( \vect y ) - \underline f$, thereby simplifying the above expression to:
   \begin{multline}\label{eq:approx_f0_inter}
      \| \vect x_{k + 1} - \vect y \|^2 \leq \| \vect x_{k} - \vect y \|^2 - \beta\lambda_k\bigl( f_0( \vect x_{k + 1 / 3} ) - f_0^* \bigr) \\
      {} + \lambda_k\rho_0( \lambda_k, k ) + \mu_k\bigl( \beta N + \rho_1( \mu_k, k ) \bigr)\text.
   \end{multline}
   Then, the boundedness of $\partial f_0( \vect x_{k} )$ leads to
   \begin{equation}\label{eq:from_f0_xk_bound}
      f_0( \vect x_{k + 1 / 3} ) \geq f( \vect x_{k} ) - M\| \vect x_{k + 1 / 3} - \vect x_{k} \|\text,
   \end{equation}
   which together with~\eqref{eq:approx_f0_inter} gives
   \begin{multline}\label{eq:approx_f0}
      \| \vect x_{k + 1} - \vect y \|^2 \leq \| \vect x_{k} - \vect y \|^2 - \beta\lambda_k\bigl( f_0( \vect x_{k} ) - f_0^* \bigr) \\
      {} + \lambda_k\bigl( \rho_0( \lambda_k, k ) + \beta M\| \vect x_{k + 1 / 3} - \vect x_{k} \| \bigr) + \mu_k\bigl( \beta N + \rho_1( \mu_k, k ) \bigr)\text.
   \end{multline}

   We shall denote, for $\delta \geq 0$:
   \begin{equation}
      X_1^\delta := \{ \vect x_k : f_0( \vect x_k ) \leq f_0^* + \delta \}.
   \end{equation}
   Notice that if $X_1$ is bounded (or $\{ \vect x_{k} \}$ is bounded), then $X_1^\delta$ is bounded. Therefore, the following quantity is well defined:
   \begin{equation}
      \Delta_1( \delta ) := \sup_{\vect x \in X_1^\delta} d_{X_1}( \vect x )\text.
   \end{equation}
   Furthermore, we have
   \begin{equation}
      \lim_{\eta \to 0} \Delta_1( \delta + \eta ) = \Delta_1( \delta )\quad\text{and}\quad \Delta_1( 0 ) = 0\text.
   \end{equation}

   Let $\delta$ be any positive real number and consider, with $\rho_0( \mu_k, k ) \leq \overline\rho_1$, $\mu_k/\lambda_k \to 0$, $\| \vect x_{k + 1 / 3} - \vect x_{k} \| \to 0$, and $\rho_0( \lambda_k, k ) \to 0$ in mind, that $k_0$ is large enough such that $k \geq k_0$ implies
   \begin{equation}\label{eq:smallness_f0}
      \rho_0( \lambda_k, k ) + \beta M\| \vect x_{k + 1 / 3} - \vect x_{k} \| < \beta\frac{\delta}{3}, \quad\text{and}\quad
      \frac{\mu_k}{\lambda_k}\bigl( \beta N + \rho_1( \mu_k, k ) \bigr) < \beta\frac{\delta}{3}\text.
   \end{equation}
   Then, two situations may occur:
   \begin{enumerate}
      \item $d_{X_1}( \vect x_k ) \geq \Delta_1( \delta )$;\label{item:lemmCXcase1}
      \item $d_{X_1}( \vect x_k ) <    \Delta_1( \delta )$.\label{item:lemmCXcase2}
   \end{enumerate}

   Let us first suppose that Case~\ref{item:lemmCXcase1} holds, that is $f_0( \vect x_{k} ) - f_0^* \geq \delta$. Then, for $k \geq k_0$, from~\eqref{eq:approx_f0}~and~\eqref{eq:smallness_f0} we get:
   \begin{equation}
      \| \vect x_{k + 1} - \vect y \|^2 \leq \| \vect x_{k} - \vect y \|^2 - \beta\lambda_k\frac\delta3.
   \end{equation}
   In particular,
   \begin{equation}
      d_{X_1}( \vect x_{k + 1} )^2 \leq \| \vect x_{k + 1} - \proj_{X_1}( \vect x_k ) \|^2 \leq d_{X_1}( \vect x_k )^2 - \beta\lambda_k\frac\delta3\text.
   \end{equation}
   Therefore, since $\sum_{k = 0}^\infty\lambda_k = \infty$, there must exist an arbitrarily large $k_1 \geq k_0$ such that $d_{X_1}( \vect x_k ) < \Delta_1( \delta )$.

   Now, let us notice that, because of~\eqref{eq:propfacforte1}
   \begin{equation}\label{eq:nextdistbound}
      \begin{split}
         d_{X_1}( \vect x_{k + 1} ) &{}\leq \| \vect x_{k + 1} - \proj_{X_1}( \vect x_{k} ) \| \\
         & {}\leq \| \vect x_{k + 2 / 3} - \proj_{X_1}( \vect x_{k} ) \| \\
         & {}\leq d_{X_1}( \vect x_k ) + \| \vect x_{k} - \vect x_{k + 2 / 3} \|\text.
      \end{split}
   \end{equation}
   Given the hypothesis, we may assume that $k_0$ is large enough such that, in addition to~\eqref{eq:smallness_f0}, we have also
   \begin{equation}
      \| \vect x_{k} - \vect x_{k + 2 / 3} \| \leq \delta.
   \end{equation}
   Therefore, for $k > k_1$, there holds:
   \begin{equation}
      d_{X_1}( \vect x_{k} ) \leq \Delta_1( \delta ) + \delta.
   \end{equation}
   Since $\delta > 0$ was arbitrary and $\lim_{\delta \to 0}\Delta_1( \delta ) = 0$, the claim is proven.\qed
\end{proof}

Before providing the general convergence result, we state and prove a simple Lemma, which we will use later.

\begin{lemma}\label{lemm:dist}
   Let $\emptyset \neq Y \subset X \subset \mathbb R^n$, where $X$ and $Y$ are convex sets. Then, for every $\vect x \in \mathbb R^n$
   \begin{equation}
      d_{Y}( \vect x ) \leq d_{Y}\bigl( \proj_{X}( \vect x ) \bigr) + 2 d_{X}( \vect x )\text.
   \end{equation}
\end{lemma}

\begin{proof}
   Using the triangular inequality and the nonexpansiveness of the projection:
   \begin{equation}
      \begin{split}
         d_Y( \vect x ) & {}= \|\vect x - \proj_{Y}( \vect x )\|\\
         & {}\leq \|\vect x - \proj_{Y}\proj_{X}( \vect x )\| + \|\proj_{Y}\proj_{X}( \vect x ) - \proj_{Y}( \vect x )\|\\
         & {}\leq \|\vect x - \proj_{Y}\proj_{X}( \vect x )\| + \|\proj_{X}( \vect x ) - \vect x\|\\
         & {}\leq \|\vect x - \proj_{X}( \vect x )\| + \|\proj_{X}( \vect x ) - \proj_{Y}\proj_{X}( \vect x )\| + \|\proj_{X}( \vect x ) - \vect x\|.
      \end{split}
   \end{equation}
   This is, by the definition of distance and projection, the desired result.\qed
\end{proof}

We introduce the notation
\begin{equation}
   [ x ]_+ := \max\{ 0, x \}.
\end{equation}


% TODO:
% Comment that
% \begin{equation}
%    \frac{\lambda_k d_{X_0}( \vect x_k )}{\mu_k} \to 0
% \end{equation}
% would suffice for convergence, under mild additional subgradient boundedness condition on $f_0$. However, sequence $\{ \vect x_{k} \}$ is required to be feasible in the fast algorithm for smooth functions.

\begin{proposition}\label{prop:CX2}
   Assume $X_2 \neq \emptyset$, $X_2$ is bounded (or $\{ \vect x_{k} \}$ is bounded), that $\sum_{i = 0}^\infty \mu_k = \infty$, $\mathcal O_{f_0}$ and $\mathcal O_{f_1}$ satisfy Property~\ref{prop:propopt1}, $\lambda_k [ f_0^* - f_0( \vect x_{k + 1 / 3} ) ]_+ / \mu_k \to 0$, $d_{X_1}( \vect x_k ) \to 0$, $\| \vect x_{k} - \vect x_{k + 1 / 3} \| \to 0$, $\| \vect x_{k + 1 / 3} - \vect x_{k + 2 / 3} \| \to 0$, $\lambda_k\rho_0( \lambda_k, k ) / \mu_k \to 0$ and $\rho_1( \mu_k, k ) \to 0$. Suppose also that there exists an $M$ such that $\forall \vect z \in \bigl\{ \vect x_k, \proj_{X_0}( \vect x_k )\bigr\}$ there is $\vect v \in \partial f_0( \vect z )$ and $\vect w \in \partial f_1( \vect z )$ for which $\| \vect v \| < M$ and $\| \vect w \| \leq M$, then we have
   \begin{equation*}
      \lim_{k\to\infty}d_{X_2}( \vect x_k ) = 0\text.
   \end{equation*}
\end{proposition}

\begin{proof}
   If we use~\eqref{eq:lemmCXaux1} with $\vect y \in X_2 \subset X_1$, we get:
   \begin{multline}\label{eq:diffestX1X2}
      \| \vect x_{k + 1} - \vect y \|^2 \leq \| \vect x_{k} - \vect y \|^2 - \beta\mu_k\bigl( f_1( \vect x_{k + 2 / 3} ) - f_1( \vect y ) \bigr) \\
      {} + \lambda_k\rho_0( \lambda_k, k ) + \mu_k\rho_1( \mu_k, k ) + \beta\lambda_k[ f_0^* - f( \vect x_{k + 1 / 3} ) ]_+\text.
   \end{multline}
   Now notice that the boundedness assumption on $\partial f_1( \vect x_k )$ leads to:
   \begin{equation}\label{eq:f0bound}
         f_1( \vect x_{k} ) \geq f_1\bigl( \vect x_{k + 2 / 3} \bigr) - M\| \vect x_k - \vect x_{k + 2 / 3} \|\text.
   \end{equation}
   Then, using~\eqref{eq:f0bound} in~\eqref{eq:diffestX1X2} it is possible to obtain:
   \begin{multline}\label{eq:diffestf1Final}
      \| \vect x_{k + 1} - \vect y \|^2 \leq \| \vect x_{k} - \vect y \|^2 - \beta\mu_k\bigl( f_1( \vect x_{k} ) - f_1^* \bigr) \\
      {} + \lambda_k\rho_0( \lambda_k, k ) + \mu_k\rho_1( \mu_k, k ) + \beta\lambda_k[ f_0^* - f_0( \vect x_{k + 1 / 3} ) ]_+ + \beta\mu_kM\| \vect x_{k + 2 / 3} - \vect x_{k} \|\text.
   \end{multline}

   Similarly to the $\Delta_1$ notation introduced above, we will denote, for $\delta \geq 0$:
   \begin{equation}
      X_2^\delta := \{ \vect x_k : f_1\bigl( \proj_{X_1}( \vect x_{k} ) \bigr) \leq f_1^* + \delta \}.
   \end{equation}
   Notice that if $X_2$ is bounded (or $\{ \vect x_{k} \}$ is bounded) and $d_{X_1}( \vect x_{k} )$ is also bounded, then $X_2^\delta$ is bounded. Therefore, the following quantity is well defined:
   \begin{equation}
      \Delta_2( \delta ) := \sup_{\vect x \in X_2^\delta} d_{X_2}( \vect x )\text.
   \end{equation}
   Furthermore, we have
   \begin{equation}
      \lim_{\eta \to 0} \Delta_2( \delta + \eta ) = \Delta_2( \delta )\quad\text{and}\quad \Delta_2( 0 ) = 0\text.
   \end{equation}

   Given the hypothesis, for any fixed $\delta > 0$, there is $k_0$ such that $k \geq k_0$ implies that
   \begin{multline}\label{eq:smallness_f1}
      \frac{\lambda_k\rho_0( \lambda_k, k )}{\mu_k} < \beta\frac{\delta}{5}, \quad
      \rho_1( \mu_k, k ) < \beta\frac{\delta}{5}, \quad
      \frac{\lambda_k[ f_0^* - f( \vect x_{k + 1 / 3} ) ]_+}{\mu_k} < \frac{\delta}{5},\\
      \text{and} \quad \mu_kM\| \vect x_{k + 2 / 3} - \vect x_{k} \| < \frac{\delta}{5}\text.
   \end{multline}

   We from now on assume $k > k_0$ and split in two different possibilities:
   \begin{enumerate}
      \item $f_1( \vect x_k ) >    f_1^* + \delta$;\label{case:lemmX2_1}
      \item $f_1( \vect x_k ) \leq f_1^* + \delta$.\label{case:lemmX2_2}
   \end{enumerate}

   We start by analyzing Case~\ref{case:lemmX2_1}. Using~\eqref{eq:smallness_f1} in~\eqref{eq:diffestf1Final} we get, for $\vect y \in X_2$:
   \begin{equation}
      \| \vect x_{k + 1} - \vect y \|^2 < \| \vect x_{k} - \vect y \|^2 - \beta\mu_k\frac\delta5.
   \end{equation}
   In particular:
   \begin{equation}
      d_{X_2}( \vect x_{k + 1} )^2 \leq \| \vect x_{k + 1} - \proj_{X_2}( \vect x_k ) \|^2 < d_{X_2}( \vect x_{k} )^2 - \beta\mu_k\frac\delta5.
   \end{equation}
   This inequality means that there is an arbitrarily large $k_1$ such that $f_1( \vect x_{k_1} ) \leq f_1^* + \delta$.

   Let us then focus on Case~\eqref{case:lemmX2_2}. We first notice that the assumed boundedness of $\partial f_1\bigl( \proj_{X_1}( \vect x_k ) \bigr)$ leads to
   \begin{equation}
      f_1\bigl( \proj_{X_1}( \vect x_k ) \bigr) \leq f_1( \vect x_k ) + Md_{X_1}( \vect x_k ).
   \end{equation}
   Therefore, $f_1( \vect x_k ) \leq f_1^* + \delta$ implies
   \begin{equation}
      \vect x_{k} \in X_2^{\delta + Md_{X_1}( \vect x_k )}.
   \end{equation}
   Thus,~\eqref{eq:nextdistbound} now reads
   \begin{equation}
      d_{X_2}( \vect x_{k + 1} ) \leq \Delta_2\bigl( \delta + Md_{X_1}( \vect x_k ) \bigr) + \| \vect x_{k + 2 / 3} - \vect x_{k} \|.
   \end{equation}

   Then, because we have assumed $d_{X_1}( \vect x_k ) \to 0$, $\| \vect x_{k} - \vect x_{k + 1 / 3} \| \to 0$, and $\| \vect x_{k + 1 / 3} - \vect x_{k + 2 / 3} \| \to 0$, we can recall $\lim_{\eta \to 0}\Delta_2( \delta + \eta ) = \Delta_2( \delta )$, so that the argumentation above leads to the conclusion that
   \begin{equation}
      \limsup_{k \to \infty}d_{X_2}( \vect x_k ) \leq \Delta_2( \delta ).
   \end{equation}
   Finally, because $\delta > 0$ was arbitrary and $\lim_{\delta \to 0} \Delta_2( \delta ) = 0$, we have just proven the claimed result.\qed
\end{proof}

We now present three different algorithms and prove their convergence, based on the above general results. Next Section contains numerical experimentation regarding some of these methods in four different bilevel models arising in high-resolution micro-tomographic image reconstruction from synchrotron illumination.

\subsection{An Algorithm for Lipschitz-Differentiable Inner Objective Functions}

In this Section we suppose $f_0$ in the bilevel optimization problem~\eqref{eq:bilevel} is differentiable with uniformly bounded and Lipschitz continuous gradient. For this kind of problem, we will consider Algorithm~\ref{algo:fiba}, which we name Fast Iterative Bilevel Algorithm (\textsc{fiba}). \textsc{fiba} first performs a projected gradient descent step, with a stepsize that does not change unless the magnitude of this operation is larger than a control sequence. This computation is then followed by the application of an optimality operator of the kind described by Properties~\ref{prop:propopt1}~and~\ref{prop:propoptbound}. The optimality operator is actually applied to a perturbation of the point obtained by the projected gradient descent, in a fashion similar to the Fast Iterative Soft-Thresholding Algorithm (\textsc{fista})~\cite{bet09}, but with the magnitude of the perturbation bounded by $\mu_k\zeta_k$, where $\{ \zeta_k \}$ is a positive vanishing sequence.

\begin{figure}
   \begin{algorithmic}[1]
      \Require{$\vect x_{0}$, $\{\lambda_k\}$, $\{\mu_k\}$, $\{\zeta_k\}$}%
      \Statex%
      \State{Initialization: $k \leftarrow 0$, $t_0 = 1$, $\vect x_{-2 / 3} = \vect x_{0}$, $i_0 = 0$ }%
      \Statex%
      \Repeat% \Comment{Main Loop}
         \Statex%
         \State{$\vect x_{k + 1 / 3} = \proj_{X_0}\bigl( \vect x_k - \lambda_{i_k}\nabla f_0( \vect x_k ) \bigr)$}\label{line:bifaStep1}% \Comment{Inner operator}
%          \Statex%
         \If{$\| \vect x_k - \vect x_{k + 1 / 3} \| \geq \zeta_k$}\label{line:bifaStep2}% \Comment{Inner operator stepsize adjustment}%
            \State{$i_{k + 1} = i_{k} + 1$}%
         \Else%
            \State{$i_{k + 1} = i_{k}$}%
         \EndIf\label{line:bifaStep3}%z
         \Statex%
         \State{$t_{k + 1} = \frac{1 + \sqrt{ 1 + 4t_{k}^2 }}{2}$, $\xi_k = \min\left\{ 1, \frac{\mu_k\zeta_k}{\| \vect x_{k + 1 / 3} - \vect x_{( k - 1 ) + 1 / 3} \|} \right\}$}%
         \State{$\vect y_{k + 1 / 3} = \vect x_{k + 1 / 3} + \xi_k\left( \frac{t_{k} - 1}{t_{k + 1}} \right)( \vect x_{k + 1 / 3} - \vect x_{( k - 1 ) + 1 / 3} )$}%
         \Statex%
         \State{$\vect x_{k + 2 / 3} = \mathcal O_{f_1}( \vect y_{k + 1 / 3}, \mu_k )$}%
         \State{$\vect x_{k + 1} = \proj_{X_0}( \vect x_{k + 2/ 3} )$}%
         \Statex%
         \State{$k \leftarrow k + 1$}%
         \Statex%
      \Until{convergence is reached}
   \end{algorithmic}
   \caption{Fast Iterative Bilevel Algorithm}\label{algo:fiba}
\end{figure}

In order to analyze convergence of Algorithm~\ref{algo:fiba} through our previous results, we first look at the simple projected gradient descent
\begin{equation}
   \mathcal G_f( \lambda, \vect x ) := \proj_{X_0}\bigl( \vect x - \lambda \nabla f( \vect x ) \bigr)
\end{equation}
as an instance of the optimality operators considered above. Let $L_f$ denote the Lipischtz constant of $\nabla f$. Then, if $\lambda \leq 1 / L_f$, it is possible to show (see, e.g., \cite{bet09} and references therein) that
\begin{equation}\label{eq:upperBoundLips}
   f( \vect y ) \leq f( \vect x ) + \nabla f( \vect x )^T( \vect y - \vect x ) + \frac 1{2\lambda}\|\vect y - \vect x \|^2.
\end{equation}
Let now $\iota_{X_0}$ be the indicator function:
\begin{equation}\label{eq:iota}
   \iota_{X_0}( \vect x ) :=
      \begin{cases}
         \infty & \text{if} \quad \vect x \notin X_0\\
         0      & \text{if} \quad \vect x \in X_0\text.
      \end{cases}
\end{equation}
Then, if $\vect y \in X_0$, inequality~\eqref{eq:upperBoundLips} leads to
\begin{equation}
   f( \vect y ) + \iota_{X_0}( \vect y ) \leq f( \vect x ) + \nabla f( \vect x )^T( \vect y - \vect x ) + \frac 1{2\lambda}\|\vect y - \vect x \|^2 + \iota_{X_0}( \vect x ).
\end{equation}
Therefore,~\cite[Lemma~2.3]{bet09} can be used with $L = 1 / \lambda$, $g = \iota_{X_0}$, $\mathbf y = \vect x$ and $\mathbf x = \vect y$ in order to get:
\begin{equation}\label{eq:fibaopt}
   \begin{split}
      2\lambda\Bigl( f( \vect y ) - f\bigl( \mathcal G_f( \lambda, \vect x ) \bigl) \Bigr) & {}\geq \| \vect x - \mathcal G_f( \lambda, \vect x ) \|^2 + 2( \vect x - \vect y )^T\bigl( \mathcal G_f( \lambda, \vect x ) - \vect x \bigr) \\
      & {} = \| \vect y - \mathcal G_f( \lambda, \vect x ) \|^2 - \| \vect y - \vect x \|^2.
   \end{split}
\end{equation}
Thus, for $\lambda \leq 1/L_f$, we can see that $\mathcal G_f( \lambda, \vect x )$ satisfies Property~\ref{prop:propopt1} with $\beta = 2$ and $\rho( \lambda, k ) \equiv 0$. Notice that the operation described at line~\ref{line:bifaStep1} of Algorithm~\ref{algo:fiba} is actually:
\begin{equation}
   \vect x_{k + 1 / 3} = \mathcal G_{f_0}( \lambda_{i_k}, \vect x_k ).
\end{equation}
Consequently, according to~\eqref{eq:fibaopt}, Algorithm~\ref{algo:fiba} is an instance of~\eqref{eq:algo} with an optimality operator $\mathcal O_{f_0}$ which satisfies Property~\ref{prop:propopt1} with $\rho_0( \lambda, k ) \equiv 0$, whenever $\lambda \leq 1 / L_f$ or if, which is weaker, \eqref{eq:upperBoundLips} holds with $\vect x = \vect x_{k}$ and $\vect y = \vect x_{k + 1 / 3}$.

Now, let us recall that $\vect x_{k} \in X_0$, so that by the definition of $\mathcal G_f$ and~\eqref{eq:propfacforte1}
\begin{equation}\label{eq:gradBoundDiff}
   \| \vect x_{k} - \mathcal G_f( \vect x_k, \lambda ) \| \leq \lambda\| \nabla f( \vect x_k ) \|.
\end{equation}
Therefore, if the sequence $\{ \nabla f_0( \vect x_{k} ) \}$ is bounded, and if $\lambda_k \to 0$ and $\zeta_k \to 0$, then the procedure in lines~\ref{line:bifaStep2}--\ref{line:bifaStep3} of Algorithm~\ref{algo:fiba} implies that $\| \vect x_{k + 1 / 3} - \vect x_{k} \| \to 0$. Observe also that if $\sum_k\lambda_k = \infty$, then $\sum_k\lambda_{i_k} = \infty$ too.

Now, we consider the fact that the optimization operator for the outer function $f_1$ is used in a perturbed point $\vect y_{k + 1 / 3}$, instead of at $\vect x_{k + 1 / 3}$. Our goal is to verify that the relevant properties of $\mathcal O_{f_1}$ are maintained. The first observation is that, given the way that $\vect y_{k + 1 / 3}$ is defined, we have
\begin{equation}\label{eq:boundmuzeta}
   \| \vect x_{k + 1 / 3} - \vect y_{k + 1 / 3} \| \leq \mu_k\zeta_k.
\end{equation}
We then define a new operator $\tilde{\mathcal O}_{f_1}$, based on $\mathcal O_{f_1}$, as follows:
\begin{equation}
   \tilde{\mathcal O}_{f_1}( \mu, \vect x_{k + 1 / 3} ) := \mathcal O_{f_1}( \mu, \vect y_{k + 1 / 3} ).
\end{equation}
Let us then assume that Property~\ref{prop:propopt1} holds for $O_{f_1}$, therefore:
\begin{equation}\label{eq:boundtildeo}
   \begin{split}
      \| \vect y - \tilde{\mathcal O}_{f_1}( \mu_k, \vect x_{k + 1 / 3} ) \|^2 & {}= \| \vect y - \mathcal O_{f_1}( \mu_k, \vect y_{k + 1 / 3} ) \|^2\\
      &{} \leq \| \vect y - \vect y_{k + 1 / 3} \|^2 - 2\mu_k\bigl( f( \mathcal O_{f_1}( \mu_k, \vect y_{k + 1 / 3} ) ) - f( \vect y ) \bigr)\\
      & \qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\quad {}+ \mu_k\rho_1( \mu_k, k )\\
      &{} = \| \vect y - \vect y_{k + 1 / 3} \|^2 - 2\mu_k\bigl( f( \tilde{\mathcal O}_{f_1}( \mu_k, \vect x_{k + 1 / 3} ) ) - f( \vect y ) \bigr)\\
      & \qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\quad {}+ \mu_k\rho_1( \mu_k, k ).\\
   \end{split}
\end{equation}
Now, by taking~\eqref{eq:boundmuzeta} into consideration, a straightforward computation leads to
\begin{equation}
   \| \vect y - \vect y_{k + 1 / 3} \|^2 \leq \| \vect y - \vect x_{k + 1 / 3} \|^2 + \mu_k\zeta_k\left( 2\| \vect y -\vect x_{k + 1 / 3} \| + \mu_k\zeta_k \right).
\end{equation}
Then, using the above bound in~\eqref{eq:boundtildeo} we have:
\begin{multline}\label{eq:prop1fromprop1}
   \| \vect y - \tilde{\mathcal O}_{f_1}( \mu_k, \vect x_{k + 1 / 3} ) \|^2 \leq \| \vect y - \vect y_{k + 1 / 3} \|^2 - 2\mu_k\bigl( f( \tilde{\mathcal O}_{f_1}( \mu_k, \vect x_{k + 1 / 3} ) ) - f( \vect y ) \bigr)\\
   {}+ \mu_k\bigl( \rho_1( \mu_k, k ) + \zeta_k( 2\| \vect y -\vect x_{k + 1 / 3} \| + \mu_k\zeta_k ) \bigr).
\end{multline}
That is, $\tilde{\mathcal O}_{f_1}$ satisfies Property~\ref{prop:propopt1} with $\rho_1$ replaced by
\begin{equation}
   \tilde\rho_1( \mu_k ,k ) := \rho_1( \mu_k, k ) + \zeta_k( 2\| \vect y -\vect x_{k + 1 / 3} \| + \mu_k\zeta_k).
\end{equation}


Given the above considerations, we are ready to provide the convergence results for Algorithm~\ref{algo:fiba}.
\begin{theorem}\label{theo:convFIBA}
   Assume $f_0$ is differentiable with Lipschitz-continuous gradient and has Lipschitz constant $L_0$. Suppose too that  $f_0$ has a bounded gradient and that $f_1$ has a bounded subgradient and $\{ f_1( \vect x_{k + 1 / 3} ) \}$ bounded from below. Assume $\{ \lambda_k \}$, $\{ \mu_k \}$ and $\{ \zeta_k \}$ are non-negative vanishing scalar sequences such that $\sum_{k = 0}^\infty \lambda_k = \infty$, $\lambda_k \leq 1/L_0$ (or each $\lambda_{i_k}$ satisfies~\eqref{eq:upperBoundLips}), $\sum_{k = 0}^\infty \mu_k = \infty$ and $\mu_k / \lambda_k \to 0$. Then, if $X_2 \neq \emptyset$, $\{\vect x_k\}$ is bounded, and $\mathcal O_{f_1}$ satisfies Properties~\ref{prop:propopt1}~and~\ref{prop:propoptbound} we have
   \begin{equation*}
      \lim_{k \to \infty} d_{X_2}( \vect x_k ) = 0.
   \end{equation*}
\end{theorem}
\begin{proof}
   First let us notice that Algorithm~\ref{algo:fiba} can be written as
   \begin{equation}%\label{eq:algo}
      \begin{split}
         \vect x_{k + 1 / 3} &{}:= \mathcal{G}_{f_0}( {\tilde\lambda}_k, \vect x_k )\text;\\
         \vect x_{k + 2 / 3} &{}:= \tilde{\mathcal{O}}_{f_1}( \mu_k, \vect x_{k + 1 / 3} )\text;\\
         \vect x_{k + 1} &{}:= \mathcal{P}_{X_0}( \vect x_{k + 2 / 3} )\text,
      \end{split}
   \end{equation}
   where ${\tilde\lambda}_k := \lambda_{i_k}$. Since the construction of the algorithm guarantees that $i_k \leq k$, we have $\sum_{k = 0}^\infty {\tilde\lambda}_k = \infty$ and $\mu_k / {\tilde\lambda}_k \to 0$. Because ${\tilde\lambda_k} \leq 1/L_0$, \eqref{eq:fibaopt} holds and therefore, $\mathcal G_{f_0}$ satisfies Property~\ref{prop:propopt1} with $\rho_0( {\tilde\lambda}_k, k ) \equiv 0$. Furthermore, because~\eqref{eq:gradBoundDiff} and the algorithm definition, as already argued, we have $\| \vect x_{k} - \vect x_{k + 1 / 3} \| \to 0$. Also, if $\mathcal O_{f_1}$ satisfies Property~\ref{prop:propoptbound} so does ${\tilde{\mathcal O}}_{f_1}$, therefore, because of the assumed subgradient boundedness and $\mu_k \to 0$ we have that $\| \vect x_{k + 1 / 3} - \vect x_{k + 2 / 3} \| \to 0$. Furthermore, as shown above, if $\mathcal O_{f_1}$ satisfies Property~\ref{prop:propopt1} so does ${\tilde{\mathcal O}}_{f_1}$, with the error term given by the factor multiplying $\mu_k$ in the second line of~\eqref{eq:prop1fromprop1}. Thus, the assumed boundedness of $\{ \vect x_k \}$ and of $f_1$ ensure that Proposition~\ref{prop:CX} can be applied so that
   \begin{equation}
      \lim_{k \to \infty} d_{X_1}( \vect x_k ) = 0.
   \end{equation}

   Now, because $\vect x_{k + 1 / 3} \in X_0$, we then have $f_0( \vect x_{k + 1 / 3} ) \geq f_0^*$. Furthermore, because of the boundedness assumptions and of $\mu_k \to 0$, it is possible to see that $\tilde\rho_1( \mu_k, k ) \to 0$. Therefore, Proposition~\ref{prop:CX2} can be applied, which leads to the desired conclusion.\qed
\end{proof}

\subsection{Incremental Algorithms for Non-Differentiable Problems}

Here we specialize Algorithm~\eqref{eq:algo} to the case where $f_0$ is the sum of several non-differentiable convex functions:
\begin{equation}
   f_0 := \sum_{i = 1}^m f_0^i.
\end{equation}
In this situation we propose the use, for the inner optimization problem, of the incremental subgradient operator, denoted as $\mathcal I_f : \mathbb R^n \times \mathbb R \to \mathbb R^n$, given by:
\begin{equation}
   \begin{split}
      \vect x^{(1)} & {}= \vect x\\
      \vect x^{(i + 1)} & {}= \vect x^{( i )} - \lambda\tilde\nabla f^i( \vect x^{(i)} )\quad i = 1, 2, \dots, m\\
      \mathcal I_f( \lambda, \vect x ) &{}= \vect x^{( m + 1 )}.
   \end{split}
\end{equation}

Incremental operators are well known for its fast initial convergence rate and, accordingly, several variations of it have been thoroughly analyzed in the literature~\cite{soz98,sol98,neb01,bhg07,dey01,bet00,ber97}. We will use here the result~\cite[Lemma~2.1]{neb01}:
\begin{lemma}\label{lemm:incsub}
   Assume the subgradients of the convex functions $f_0^i$ are bounded in the following sense:
   \begin{equation}\label{eq:subgradBoundInc}
      \forall \vect x \in \mathbb R^n\quad\text{and}\quad \forall\vect v \in \partial f_0^i( \vect x ), \quad \| \vect v \| \leq C_i, \quad i\in \{1, 2, \dots, m\}.
   \end{equation}
   Then, the incremental subgradient operator satisfies, for every $\lambda \in \mathbb R_+$, and $\vect y, \vect x \in \mathbb R^n$:
   \begin{equation}\label{eq:incsub}
      \| \mathcal I_{f_0}( \lambda, \vect x ) - \vect y \|^2 \leq \| \vect x - \vect y \|^2 - 2\lambda \bigl( f_0( \vect x ) - f_0( \vect y ) \bigr) + \lambda^2\bigl( \sum_{i = 1}^mC_i \bigr)^2\text,
   \end{equation}
   where $f_0 := \sum_{i = 1}^m f_0^i$.
\end{lemma}

Now, noticing that
\begin{equation}\label{eq:incsubbound}
   \| \mathcal I_{f_0}( \lambda, \vect x ) - \vect x \| \leq \lambda\sum_{i = 1}^m C_i
\end{equation}
and applying Proposition~\ref{prop:oneIsOther} we are lead to the following result:
\begin{corollary}
   Assume the subgradients of the convex functions $f_0^i$ satisfy~\eqref{eq:subgradBoundInc}. Then, the incremental subgradient operator satisfies, for every $\lambda \in \mathbb R_+$, and $\vect y, \vect x \in \mathbb R^n$:
   \begin{equation}
      \| \mathcal I_{f_0}( \lambda, \vect x ) - \vect y \|^2 \leq \| \vect x - \vect y \|^2 - 2\lambda \bigl( f_0\bigl( \mathcal I_{f_0}( \lambda, \vect x ) \bigr) - f_0( \vect y ) \bigr) + \lambda^2K\text,
   \end{equation}
   where $K = \bigl( \sum_{i = 1}^mC_i \bigr)^2 + 2\bigl( \sum_{i = 1}^mC_i \bigr)^{3/2}$ and, again, $f_0 := \sum_{i = 1}^m f_0^i$.
\end{corollary}

The second algorithm we propose in this work will be called \textsc{iiba}, from Incremental Iterative Bilevel Algorithm, and is described in Algorithm~\ref{algo:iiba} below. For this algorithm we have the following convergence result.

\begin{figure}
   \begin{algorithmic}[1]
      \Require{$\vect x_{0}$, $\{\lambda_k\}$, $\{\mu_k\}$}%
      \Statex%
      \State{Initialization: $k \leftarrow 0$}%
      \Statex%
      \Repeat% \Comment{Main Loop}
         \Statex%
         \State{$\vect x_{k + 1 / 3} = \mathcal I_{f_0}( \vect x_k )$}\label{line:iifaStep1}% \Comment{Inner operator}
         \State{$\vect x_{k + 2 / 3} = \mathcal O_{f_1}( \vect y_{k + 1 / 3}, \mu_k )$}%
         \State{$\vect x_{k + 1} = \proj_{X_0}( \vect x_{k + 2/ 3} )$}%
         \State{$k \leftarrow k + 1$}%
         \Statex%
      \Until{convergence is reached}
   \end{algorithmic}
   \caption{Incremental Iterative Bilevel Algorithm}\label{algo:iiba}
\end{figure}

\begin{theorem}\label{theo:convIIBA}
   Assume that $f_0$ is of the form $f_0 := \sum_{i = 1}^m f_0^i$ and satisfies~\eqref{eq:subgradBoundInc}, that $f_1$ has a bounded subgradient, and that $\{ f_1( \vect x_{k + 1 / 3} ) \}$ is bounded from below. Assume $\{ \lambda_k \}$ and $\{ \mu_k \}$ are non-negative vanishing scalar sequences such that $\sum_{k = 0}^\infty \lambda_k = \infty$, $\sum_{k = 0}^\infty \mu_k = \infty$, $\mu_k / \lambda_k \to 0$ and $\lambda_k^2 / \mu_k \to 0$. Then, suppose $X_2 \neq \emptyset$ and $X_2$ is bounded (or $\{\vect x_k\}$ is bounded), and $\mathcal O_{f_1}$ satisfies Properties~\ref{prop:propopt1}~and~\ref{prop:propoptbound} with $\rho_1( \mu_k ,k ) \to 0$. Then, the sequence $\{ \vect x_k \}$ generated by Algorithm~\ref{algo:iiba} satisfies
   \begin{equation*}
      \lim_{k \to \infty} d_{X_2}( \vect x_k ) = 0.
   \end{equation*}
\end{theorem}
\begin{proof}
   Notice that Lemma~\ref{lemm:incsub} together with Proposition~\ref{prop:oneIsOther} and the subgradient boundedness assumption imply that $\mathcal I_{f_0}$ satisfies the desired Property~\ref{prop:propopt1}. Also, $\lambda_k \to 0$ implies, together with the subgradient boundedness assumption, that $\| \vect x_k - \vect x_{k + 1/3} \| \to 0$ and that $\rho_0( \lambda_k, k ) \to 0$, the latter because of Lemma~\ref{lemm:incsub}. Also, Property~\ref{prop:propoptbound} of $\mathcal O_{f_1}$ together with $\mu_k \to 0$ imply that $\| \vect x_{k + 1 / 3} - \vect x_{k + 2 / 3} \| \to 0$. Therefore, Proposition~\ref{prop:CX} implies that
   \begin{equation}
      d_{X_1}( \vect x_k ) \to 0.
   \end{equation}

   Now, notice the subgradient boundedness assumption and~\eqref{eq:incsubbound} imply that $[ f_0( \vect x_k ) - f_0( \vect x_{k + 1 / 3} ) ]_+  = O( \lambda_k )$, and, therefore, since $\vect x_k \in X_0$ for $k > 0$, we have $[ f_0^* - f( \vect x_{k + 1 / 3} ) ]_+  = O( \lambda_k )$. Thus, $\lambda_k^2 / \mu_k \to 0$ implies $\lambda_k[ f_0^* - f( \vect x_{k + 1 / 3} ) ]_+ / \mu_k \to 0$. Furthermore, since, by~\eqref{eq:incsub}, $\rho_0( \lambda_k, k ) = O( \lambda_k )$, $\lambda_k^2 / \mu_k$ also implies $\lambda_k\rho_0( \lambda_k, k ) / \mu_k \to 0$. So, finally, Proposition~\ref{prop:CX2} can be applied, which proves the result.\qed

\end{proof}

\subsection{Stopping Criterion}

Here we devise a stopping criterion for the 

\section{Numerical Experimentation}

\subsection{Problem Presentation}

We have performed experiments involving tomographic image reconstruction. In tomography, the idealized problem is to reconstruct a function $g : \mathbb R^2 \to \mathbb R$ given the values of its integrals along straight lines, that is, given its \emph{Radon transform} denoted as $\mathcal R[ g ]$ and defined by the following equality:
\begin{equation}
   \mathcal R[ g ]( \theta, t ) := \int_{\mathbb R} g\left( t\left(\begin{smallmatrix}\cos\theta\\ \sin\theta\end{smallmatrix}\right) + s \left(\begin{smallmatrix}-\sin\theta\\ \cos\theta\end{smallmatrix}\right)\right) \mathrm ds.
\end{equation}
Figure~\ref{fig:rad} (adapted from~\cite{hcc14}) brings a graphical representation of this definition.

\begin{figure}
   \centering%
   \input{sl.tex}%
   \input{figradonteta.tex}%
   \def\tlinha{-0.6}%
   \setlength{\grftotalwidth}{0.45\columnwidth}%
   \setlength{\grfticksize}{0.5\grfticksize}%
   \small{\ }\hfill%
   \begin{grfgraphic}{%
      \def\grfxmin{-2.05}\def\grfxmax{1.5}%
      \def\grfymin{-1.5}\def\grfymax{2.05}%
   }%
      \begin{scope}[>=stealth,style=grfaxisstyle,<->]%
         %Phantom:
         \shepplogan%
         %Eixos:
         \draw (-1.5,0) -- (1.5,0);%
         \draw (0,-1.5) -- (0,1.5);%
         \foreach \i in {-1,1}%
         {
            \draw[style=grftickstyle,-] (\i\grfxunit,-\grfticksize) -- (\i\grfxunit,\grfticksize);%
            \draw[style=grftickstyle,-] (-\grfticksize,\i\grfyunit) -- (\grfticksize,\i\grfyunit);%
         }
         \begin{scope}[rotate=\teta]
            \draw (-1.5,0) -- (1.5,0);
            \foreach \i in {-1,1}
               \draw[style=grftickstyle,-] (\i\grfxunit,-\grfticksize) -- (\i\grfxunit,\grfticksize);
            %Caminho de integração:
            \draw[dashed,dash phase=-0.005\grfyunit] (\tlinha,-1.5) -- (\tlinha,1.5);
            \fill (\tlinha,0) node[anchor=north,inner sep=\grflabelsep] {\scriptsize$t$} circle (0.025cm);
            %Perpendicular:
            \draw[-] (\tlinha\grfxunit,0.3em) -| (\tlinha\grfxunit - 0.3em,0pt);
            \fill (\tlinha\grfxunit - 0.15em,0.15em) circle (0.025cm);
         \end{scope}
         \begin{scope}[rotate=\teta,yshift=1.5\grfyunit]
            %Gráfico:
            \draw[line width=0.025cm] plot file {figradon.data};
            \draw[-]  (1.5,0) -- (-1.5,0) node[anchor=north,rotate=\teta,inner sep=\grflabelsep] {\scriptsize$t$};
            \draw[->] (0,0)    -- (0,0.7) node[anchor=west,rotate=\teta,inner sep=\grflabelsep]  {\scriptsize$\mathcal R[ \mu ](\theta,t)$};
         \end{scope}
         %Trabalho extra para evitar bug em \tikz \arc ao desenhar o ângulo:
         \def\rad{0.075}
         \FPupn{\cpt}{0.552285 \rad{} * 90 \teta{} / *}
         \path (\teta:\rad) ++(\teta - 90:\cpt) node (a) {};
         \draw[-] (0,0) -- (\rad,0) .. controls +(0,\cpt) and (a) .. (\teta:\rad) -- cycle;
         \draw[style=grftickstyle,-,rotate=\tetameio,xshift=\rad\grfxunit] (-\grfticksize,0pt) -- (\grfticksize,0pt);
         \path[rotate=\tetameio,xshift=0.3em] (\rad,0) node[anchor=west,inner sep=0pt] {\scriptsize$\theta$};
      \end{scope}
   \end{grfgraphic}\hfill%
   \begin{grfgraphic}[1.125]{%
      \grfyaxis[R]{[]-1;0;1[]}{[]\tiny$-1$;\tiny$0$;\tiny$1$[]}%
      \grfylabel{\footnotesize$t$}%
      \grfxaxis[R]{[]0;1.57;3.14[]}{[]\tiny$0$;\tiny$\frac\pi2$;\tiny$\pi$[]}%
      \grfxlabel{\footnotesize$\theta$}%
      \def\grfxmin{0}%
      \def\grfxmax{3.14}%
      \grfwindow%
   }%
      \node[anchor=north west,inner sep=0pt] at (0,1)
      {\includegraphics[width=3.14\grfxunit,height=2\grfyunit]
      {figrad_sino}};%
   \end{grfgraphic}\hfill{\ }%
   \caption{Left: schematic representation of the Radon transform. In
   the definition, $\theta$ is the angle between the normal to
   the integration path and the horizontal axis, while $t$ is the
   the line of integration's displacement from the origin.
   Right: Image of the Radon transform of the image shown on the
   left in the $\theta \times t$ coordinate system.}\label{fig:rad}%
\end{figure}

We have used both synthetic and real data in our numerical essays. Synthetic data was noise-free and ideally discretized, leading to the possibility of exact reconstruction of the original image. Real data was obtained by transmitting synchrotron radiation through samples of eggs taken from a fish of the species \emph{Prochilodus lineatus} collected at the Madeira River`s bed, immersed in distilled water inside a capillary test tube. Data acquisition was performed at the Brazilian National Synchrotron Light Source (\textsc{lnls})\footnote{\url{http://lnls.cnpem.br/}}.

In a transmission tomography setup~\cite{kas88,nat86,her80} like the one we have used, the value of the line integral is estimated through the emitted to detected intensity ratio according to Beer--Lambert law:
\begin{equation}
   \frac{I_e}{I_d} = e^{\int_{L}g( \vect x )\mathrm ds},
\end{equation}
where $I_e$ is the emitted intensity, $I_d$ is the detected intensity, $\mu$ gives the linear attenuation factor of the imaged object at each point in space, and $L$ is the straight line connecting detector to emitter. While in this case the reconstruction problem is essentially bi-dimensional, a simultaneous acquisition of a radiography of $2048$ parallel slices of the object to be imaged is made at each angle, which enables volumetric reconstruction, if desired, by the stacking of several bi-dimensional reconstructions. After each plain \textsc{x}-ray imaging, the sample is rotated and new samples of the Radon transform are estimated in the same manner at a new angle. Figure~\ref{fig:experimental_Radon} depicts the process of assembling the $2048 \times 200$ data array, which will be used for a slice reconstruction, from the $200$ images of size $2048 \times 2048$.

In our application the imaged subject is sensitive in a way such that a overly long exposure time under a low energy \textsc{x}-ray beam may overheat or otherwise physically damage the sample. Therefore, because the exposure time for good radiographies under a monochromatic beam at LNLS' facilities was experimentally found to be at least $20$ seconds, the Radon Transform was sampled at only $200$ evenly spaced angles covering the interval $[-\pi, 0]$, a relatively small number if we are willing to reconstruct full resolution $2048 \times 2048$ images from this data. In this case, it is likely that problem~\eqref{eq:leastsq} will have many solutions and we need to select one of these, therefore the need of a bilevel model arises.

\begin{figure}
   \input{egg_illustration_data.tex}%
   \centering%
   \setlength{\grftotalwidth}{\textwidth}%
   \begin{grfgraphic}{%
      \def\grfxmin{0.0}\def\grfxmax{3.0}%
      \def\grfymin{-0.5}\def\grfymax{0.5}%
   }%
      \node[inner sep=0pt] at (0.5,0.0) {\includegraphics[width=\grfxunit]{egg_projection_0}};%
      \node[inner sep=0pt] at (1.5,0.0) {\includegraphics[width=\grfxunit]{egg_projection_1}};%
      \node[inner sep=0pt] at (2.5,0.0) {\includegraphics[width=\grfxunit]{egg_projection_2}};%
      \draw[grfaxisstyle] (0.0,-0.5) rectangle (1.0,0.5);%
      \draw[grfaxisstyle] (1.0,-0.5) rectangle (2.0,0.5);%
      \draw[grfaxisstyle] (2.0,-0.5) rectangle (3.0,0.5);%
      \draw[grfaxisstyle,red,opacity=0.5] (0.0,\sliceHeight) -- (1.0,\sliceHeight);%
      \draw[grfaxisstyle,green,opacity=0.5] (1.0,\sliceHeight) -- (2.0,\sliceHeight);%
      \draw[grfaxisstyle,blue,opacity=0.5] (2.0,\sliceHeight) -- (3.0,\sliceHeight);%
   \end{grfgraphic}\\[5pt]%
   \begin{grfgraphic}[0.6]{%
      \grfxaxis{[]0.0;1.0;2.0;3.0[]}{[]\small$0.0$;\small$-\frac\pi3$;\small$-\frac{2\pi}3$;\small$-\pi$[]}%
      \grfyaxis[r]{[]-1.0;0.0;1.0[]}{[]\small$-0.38$;\small$0.0$;\small$0.38$[]}%
   }%
      \node[inner sep=0pt] at (1.5,0.0) {\includegraphics[width=3\grfxunit,height=2\grfyunit]{egg_sino}};%
      \draw[grfaxisstyle] (0.0,-1.0) rectangle (3.0,1.0);%
      \draw[grfaxisstyle,red,opacity=0.5] (\projectionAPos,-1.0) -- (\projectionAPos,1.0);%
      \draw[grfaxisstyle,green,opacity=0.5] (\projectionBPos,-1.0) -- (\projectionBPos,1.0);%
      \draw[grfaxisstyle,blue,opacity=0.5] (\projectionCPos,-1.0) -- (\projectionCPos,1.0);%
   \end{grfgraphic}%
   \caption{Assembly of the Radon Transform. Top: three of the $200$ radiographic images used, each of which has $2048 \times 2048$ pixels and depicts a square region of area $0.76 \times 0.76$mm${^2}$. Bottom: the $n^{\text{\scriptsize th}}$ row of the $i^{\text{\scriptsize th}}$ image has samples of $\mathcal R[ g^n ]( \theta_i, \cdot )$, that is, a column in the representation of $\mathcal R[ g^n ]$ in the $\theta \times t$ plane, where $g^n : \mathbb R^2 \to \mathbb R$ gives the linear attenuation factor at each point in the $n^{\text{\scriptsize th}}$ slice to be reconstructed. The colored solid lines depict the position of the radiographies' rows in the resulting sinogram.}\label{fig:experimental_Radon}%
\end{figure}

\subsection{Inner Objection Functions}

Assuming the original image $g : \mathbb R^2 \to \mathbb R_+$ lies in a finite dimensional vector space generated by some basis $\{ g^1, g^2, \dots, g^n \}$ and recognizing that the number of measurements is always finite in practice, one can reduce the problem of tomographic reconstruction to a linear system of equations:
\begin{equation}\label{eq:linsys}
   R\vect x = \vect b,
\end{equation}
where the elements $r_{ij}$ of the matrix $R$ are given by
\begin{equation}\label{eq:linsys}
   \mathcal R[g^j]( \theta_i, t_i )
\end{equation}
and the elements $b_i$ of the vector $\vect b$ are the corresponding experimental data, that is, $b_i$ is an approximate sample of $\mathcal R[g]( \theta_i, t_i )$, where $g = \sum_{i = 1}^nx_ig^i$ is the desired image. Because actual microtomographic data from synchrotron illumination will always contain errors (either from micrometric misalignment of the experimental setup, small dust particles in the emitter-detector path, or from statistical fluctuation of photon emission and attenuation), the above linear system of equations may not have a solution.

\subsection{Differentiable Inner Objective Function}

System~\eqref{eq:linsys} can be replaced by a constrained least squares problem, in order to alleviate the likely lack of consistency:
\begin{equation}\label{eq:leastsq}
   X_1 = \argmin_{\vect x \in \mathbb R_+^n} q( \vect x ) := \frac12\| R\vect x - \vect b \|^2.
\end{equation}
Therefore, in this case we will be lead to a bilevel problem of the form~\eqref{eq:bilevel} with $X_0 = \mathbb R_+^n$.

% Because we are considering a simple feasible set, we use the orthogonal projection onto it as feasibility operator:
% \begin{equation*}
%    \mathcal F_{X_0}( \lambda, \vect x ) := \mathcal P_{\mathbb R_+^n}( \vect x ).
% \end{equation*}
% It is possible to observe that this operator satisfies the required Property~\ref{prop:propfac} with $E=0$ for any $\varepsilon > 0$.

Another option for a feasibility set would be the bounded box $\{ \vect x \in \mathbb R^n : 0 \leq x_i \leq u \}$ for some $u > 0$. This may be a sensible idea if the maximum attenuation factor is known beforehand and we could thus include this information into the model. Because we do not make this kind of boundedness imposition, by using the least squares function we are at the risk of violating certain (sub)gradient boundedness assumption. We therefore use another continuously differentiable convex function $f_0$, which has an uniformly bounded gradient and is such that
\begin{equation}\label{eq:probEquiv}
   \argmin_{\vect x \in X_0} f_0( \vect x ) = \argmin_{\vect x \in X_0} q( \vect x ).
\end{equation}
In order to build such function, take any $\tilde{\vect x} \in X_0$ (such as, in our case, $\tilde{\vect x} = \vect 0$) and set
\begin{equation}
   \Delta := \| R\tilde{\vect x} - \vect b \| > 0,
\end{equation}
then define
\begin{equation}
   f_0( \vect x ) := \frac12\sum_{i = 1}^m h( \langle r_i, \vect x \rangle - b_i ),
\end{equation}
where $r_i^T$ is the $i$-th row of $R$ and the function $h : \mathbb R \to \mathbb R_+$ is given as
\begin{equation}
   h( x ) := \begin{cases}
                      x^2 & \text{if}\quad |x| < \Delta\\
                      2\Delta|x| - \Delta & \text{otherwise.}
                   \end{cases}
\end{equation}
Notice that if $q(\vect x) \leq q( \tilde{\vect x} ) = 1/2\Delta^2$, then $f_0( \vect x ) = q( \vect x )$ and, furthermore, if $f_0( \vect x ) \neq q( \vect x )$, then $f_0( \vect x ) \geq 1/2\Delta^2 = q( \tilde{\vect x} )$. Therefore, \eqref{eq:probEquiv} holds.

We need to show that the uniformly bounded continuous differentiability and convexity claims hold, but these facts follow from convexity and continuous differentiability of $h$. Its derivative can be computed to be
\begin{equation}
   h'( x ) := \begin{cases}
                 2x & \text{if}\quad |x| < \Delta\\
                 2\Delta\sign(x) & \text{otherwise,}
              \end{cases}
\end{equation}
with $\sign : \mathbb R \to 2^{\mathbb R}$ defined as
\begin{equation}
   \sign( x ) := \begin{cases}
                     -1      & \text{if}\quad x < 0\\
                     [-1, 1] & \text{if}\quad x = 0\\
                      1      & \text{if}\quad x > 0.
                 \end{cases}
\end{equation}
Thus, the derivative of $h$ is uniformly bounded by $| h'( x ) | \leq 2\Delta$, is continuous as long as we use $\Delta > 0$, and, since $h'( x )$ is nondecreasing, $h$ is convex. Notice that $h$ is the well known Huber function~\cite{hub64}.

% \subsubsection{Inner Optimality Operator}
% 
% We define the following simple optimality operator for the inner objective function:
% \begin{equation}\label{eq:innerOp0}
%    O_{f_0}( \lambda, \vect x ) := \vect x - \lambda\nabla f_0( \vect x ).
% \end{equation}
% Using this definition together with the definition of the $2$-norm followed by the (sub)gradient inequality for convex functions leads to:
% \begin{equation}
%    \| O_{f_0}( \lambda, \vect x ) - \vect y \|^2 \leq \| \vect x - \vect y \|^2 - 2\bigl( f_0( \vect x ) - f_0( \vect y ) \bigr) + \lambda^2\| \nabla f_0( \vect x ) \|^2.
% \end{equation}
% Also, directly from definition~\eqref{eq:innerOp0} we have
% \begin{equation}
%    \| O_{f_0}( \lambda, \vect x ) - \vect x \|^2 = \lambda\| \nabla f_0( \vect z ) \|.
% \end{equation}
% Therefore, Property~\ref{prop:propopt1} is satisfied with $\beta = 2$ and $\rho_0( \lambda, k ) = \lambda K^2$ and Property~\ref{prop:propoptbound} is satisfied with $\gamma = K$, where $K$ is a bound on the norm of $\nabla f_0( \vect x )$, which, as can be deduced from equation~\eqref{eq:gradSQMod} below, is uniformly bounded.

In order to simplify the notation, we introduce the function $\vect h' : \mathbb R^m \to \mathbb R^m$ given as:
\begin{equation}
   \vect h'( \vect x ) := \left(\begin{matrix}
                                   h'( x_1 )\\
                                   h'( x_2 )\\
                                   \vdots\\
                                   h'( x_m )
                               \end{matrix}\right).
\end{equation}
Under this notation, a straightforward calculation leads to
\begin{equation}\label{eq:gradSQMod}
   \nabla f_0( \vect x ) =\frac12 R^T\vect h'( R\vect x - \vect b ).
\end{equation}
The computationally expensive parts of this expression are products of the form $R\vect x$ and $R^T\vect b$. In our case, because of image resolution and dataset size, as explained in the previous Subsection, matrix $R$ has dimensions of over $4\cdot 10^5$ lines by $4\cdot10^6$ columns.

In order to obtain a computationally viable algorithm, these matrix-vector products must be amenable to fast computation, and, in fact, there is a very effective approach to it based in a relation between the one-dimensional Fourier Transform of the data and one ``slice'' of the two-dimensional Fourier Transform of the original image. Recall that we denote our desired, unknown, image as $g : \mathbb R^2 \to \mathbb R_+$ and define the projection of $f$ at an angle $t$ as
\begin{equation*}
   p_\theta( t ) := \mathcal R[ g ]( t ).
\end{equation*}
Now, using the hat notation for the Fourier transform of an integrable function $f : \mathbb R^n \to \mathbb C$, as defined by
\begin{equation}
   \hat f( \vect \omega ) := \mathcal F[ f ]( \vect \omega ) := \int_{\mathbb R^n} f( \vect x ) e^{-i2\pi\langle \vect\omega, \vect x \rangle} \mathrm d\vect x,
\end{equation}
there holds the so called Fourier-slice theorem~\cite{kas88,nat86}:
\begin{equation}\label{eq:fourierSlice}
   \hat p_\theta( \omega ) = \hat g\left( \omega\left( \begin{smallmatrix}
                                                            \cos\theta\\
                                                            \sin\theta
                                                         \end{smallmatrix}
                                            \right)\right).
\end{equation}

This result implies that the action of $R$ can be evaluated first in the Fourier space, an operation which can be computed efficiently by Non-uniform Fast Fourier Transforms (\textsc{nfft})~\cite{fou03} and later translated back to the original feature space by regular Fast Fourier Transforms (\textsc{fft}). We have used the \texttt{pynfft} binding for the \texttt{nfft3} library~\cite{kkp09} in order to compute samples of $\hat p_\theta$ following~\eqref{eq:fourierSlice}, and then used regular inverse \textsc{fft} routines from \texttt{numpy} for the final computation from the Fourier back to the feature space. Fast evaluation of the transpose operation is immediately available from the same set of libraries using the \textsc{fft} from \texttt{numpy} and the transpose of the \textsc{nfft} available from \texttt{nfft3}.



% In order to construct our proposed optimality operator for this inner objective function $f_0$ we first consider the following, slightly more general, operation, defined for convex functions $f$:
% \begin{equation}
%    \mathcal {OF}_f( \lambda, \nu, \vect x, \vect y ) := \vect z - \lambda\tilde\nabla f( \vect z ),
% \end{equation}
% with $\lambda$ and $\nu$ nonnegative scalars, $\vect x$ and $\vect y$ in $\mathbb R^n$,
% \begin{equation}
%    \vect z := \vect x + \nu\vect y, \quad \text{and} \quad \tilde\nabla f( \vect z ) \in \partial f( \vect z ).
% \end{equation}
% Let us now perform some computations:
% \begin{equation}
%    \begin{split}
%       \| \mathcal {OF}_f( \lambda, \nu, \vect x, \vect y ) - \vect w \|^2 & {}= \| \vect z - \lambda\tilde\nabla f( \vect z ) - \vect w \|^2\\
%       & {}= \| \vect z - \vect w \|^2 - 2\lambda\langle \tilde\nabla f( \vect z ), \vect z - \vect w \rangle + \lambda^2\| \tilde\nabla f( \vect z ) \|^2\\
%       & {}\leq \| \vect z - \vect w \|^2 - 2\lambda \bigl( f( \vect z ) - f( \vect w ) \bigr) + \lambda^2\| \tilde\nabla f( \vect z ) \|^2\\
%       & {}= \| \vect x + \nu \vect y - \vect w \|^2 - 2\lambda \bigl( f( \vect z ) - f( \vect w ) \bigr) + \lambda^2\| \tilde\nabla f( \vect z ) \|^2\\
%       & {}\leq \| \vect x - \vect w \|^2 - 2\lambda \bigl( f( \vect z ) - f( \vect w ) \bigr) + \lambda^2\| \tilde\nabla f( \vect z ) \|^2 \\
%       & \quad\qquad\qquad\qquad\qquad\qquad {} + \nu^2\| \vect y \|^2 + \nu\| \vect y \|\| \vect x - \vect w \|,
%    \end{split}
% \end{equation}
% where the first two equalities are matter of definitions, the first inequality comes from the subgradient inequality, the third identity comes from the definition of $\vect z$ and the last relation is obtained by the definition of the norm followed by Cauchy-Schwartz inequality. By a simple argument based on the subgradient inequality one has $f( \vect z ) \geq f( \vect x ) - \nu\| \tilde\nabla f( \vect z ) \|\| \vect y \|$, from where we finally reach
% \begin{multline}
%    \| \mathcal {OF}_f( \lambda, \nu, \vect x, \vect y ) - \vect w \|^2 \leq \| \vect x - \vect w \|^2 - 2\lambda \bigl( f( \vect x ) - f( \vect w ) \bigr)\\
%    {}+ \lambda^2\| \tilde\nabla f( \vect z ) \|^2 + \nu^2\| \vect y \|^2 + \nu\| \vect y \|\| \vect x - \vect w \|\\
%    {}+ 2\lambda\nu\| \tilde\nabla f( \vect z ) \|\| \vect y \|.
% \end{multline}
% 
% We now define our optimality operator for the inner objective function as an iteration dependent operator, to be understood in the context of the running algorithm, where $k$ is the iteration number:
% \begin{equation}
%    \mathcal O_{f_0}( \lambda, \vect x ) := \mathcal {OF}_{f_0}\left( \lambda, \frac{\lambda}{\lambda_0}\frac{t_k - 1}{t_{k + 1}}, \vect x, \vect x - \vect x_{k} \right),
% \end{equation}
% where
% \begin{equation}
%    t_0 = 1 \quad \text{and} \quad t_{k + 1} = \frac{1 + \sqrt{1 + 4t_{k}^2}}{2}.
% \end{equation}
% Now, because the operator will always be applied at $\vect x = \vect x_{k + 1/3}$, inequality 

\subsection{Non-Differentiable Inner Objective Function}

Another option to circumvent the non-consistency of~\eqref{eq:linsys} under non-negativity constraints is to use the least 1-norm approach, which is useful because synchrotron illuminated tomographic data contains mostly very mild noise, but also has sparsely distributed high intensity noisy points possibly caused by small dust particles and other detector failures such as those caused by defective scintillator crystals and other mechanical, thermal or electronic causes~\cite{mro14}.

Therefore, our second option for inner optimization problem was given by
\begin{equation}\label{eq:leastsq}
   X_1 = \argmin_{\vect x \in \mathbb R_+^n} \ell( \vect x ) := \| R\vect x - \vect b \|_1.
\end{equation}
Where, now, the inner objective function naturally has an everywhere bounded subdifferential and, as is well known, the $\| \cdot \|_1$ is more forgiving to sparse noise than is the euclidean norm.


\subsection{Outer Objective Functions}

For the purpose of selecting one among the solutions of~\eqref{eq:leastsq}, we will consider two particular cases of the bilevel program~\eqref{eq:bilevel}.

\subsubsection{Haar 1-Norm}

Here the outer function is given by
\begin{equation}
   f_{\text{Haar}}( \vect x ) := \| H\vect x \|_1,
\end{equation}
with $H \in \mathbb R^{n \times n}$ orthonormal, that is, satisfies $H^TH = I$, where $I$ is the identity matrix and superscript $T$ indicates transposition. Transformation $H$ is usually a sparsefying transform, in our case the Haar transform, and one is looking for a sparse (in some cases the sparsest~\cite{crt06,crt06b,don06,don06b,don06c}), in the $H$-transformed space, optimizer of $f_0$ over $X_0$.

Notice that for this particular function we have
\begin{equation}\label{eq:subdiffHaar}
   \partial f_{\text{Haar}}( \vect x ) = H^T\vect\sign( H\vect x ),
\end{equation}
where the set-valued function $\vect\sign : \mathbb R^n \to 2^{\mathbb R^n}$ is given by
\begin{equation}
   \vect\sign( \vect v ) := \{ \vect x \in \mathbb R^n : x_i \in \sign( v_i ) \}.
\end{equation}

Let us now consider the soft-thresholding operator, given
componentwise as
\begin{equation}
   \bigl( \text{\textsc{st}}_\mu( \vect x ) \bigr)_i := 
      \begin{cases}
         x_i + \mu & \text{if}\quad x_i < -\mu\\
         0         & \text{if}\quad x \in [ -\mu, \mu ]\\
         x_i - \mu & \text{if}\quad x_i > \mu.
      \end{cases}
\end{equation}
We then define an intermediary optimality operator as
\begin{equation}
   \mathcal N_{f_{\text{Haar}}}( \mu, \vect x ) := H^T\text{\textsc{st}}_\mu( H\vect x ).
\end{equation}
A straightforward computation convinces us that
\begin{equation}\label{eq:HSTasSubgrad}
   \mathcal N_{f_{\text{Haar}}}( \mu, \vect x ) = \vect x - \mu \tilde\nabla f_1( \overline{\vect x} ),
\end{equation}
where
\begin{equation}
   \overline{x}_i = \begin{cases}
                        x_i - \sign( x_i )\mu & \text{if}\quad | x_i | > \mu\\
                        0   & \text{if}\quad | x_i | \leq \mu
                     \end{cases} = \mathcal N_{f_{\text{Haar}}}( \mu, \vect x ),
\end{equation}
and $\tilde\nabla f_1( \overline{\vect x} ) \in \partial f_{\text{Haar}}( \overline{\vect x} )$.
Now we proceed:
\begin{equation}\label{eq:hstDiffBound}
   \begin{split}
      \| \mathcal N_{f_{\text{Haar}}}( \mu, \vect x ) - \vect y \|^2 &{}= \| \vect x - \mu \tilde\nabla f_{\text{Haar}}( \overline{\vect x} ) - \vect y \|^2\\
      &{} = \| \vect x - \vect y \|^2 - 2\mu\langle \tilde\nabla f_{\text{Haar}}( \overline{\vect x} ), \vect x - \vect y \rangle + \| \mu \tilde\nabla f_{\text{Haar}}( \overline{\vect x} ) \|^2\\
      &{} = \| \vect x - \vect y \|^2 - 2\mu\langle \tilde\nabla f_{\text{Haar}}( \overline{\vect x} ), \overline{\vect x} - \vect y \rangle \\
      &\qquad\qquad\qquad {}- 2\mu\langle \tilde\nabla f_{\text{Haar}}( \overline{\vect x} ), \vect x - \overline{\vect x} \rangle + \| \mu \tilde\nabla f_{\text{Haar}}( \overline{\vect x} ) \|^2
   \end{split}
\end{equation}
and we then can observe from~\eqref{eq:subdiffHaar} that $\partial f_1$ is bounded in a way such that $\| \tilde \nabla f_1( \vect x ) \| \leq \sqrt n$ for every $\vect x$, and from~\eqref{eq:hstDiffBound} that $\| \vect x - \overline{\vect x} \| \leq \mu \sqrt n$ for every $\vect x$. Using this facts followed by the subgradient inequality we have
\begin{equation}\label{eq:propOptHaarSoftThres}
   \begin{split}
      \| \mathcal N_{f_{\text{Haar}}}( \mu, \vect x ) - \vect y \|^2 &{}\leq \| \vect x - \vect y \|^2 - 2\mu\langle \tilde\nabla f_{\text{Haar}}( \overline{\vect x} ), \overline{\vect x} - \vect y \rangle + 3\mu^2n\\
      &{}\leq \| \vect x - \vect y \|^2 - 2\mu\bigl( f_{\text{Haar}}( \overline{\vect x} ) - f_1( \vect y )\bigr) + 3\mu^2n.
   \end{split}
\end{equation}
% But now, again using the boundedness facts on $\partial f_1$ and $\overline{\vect x} - \vect x$ together with the subgradient inequality, we can conclude that $f_1( \overline{\vect x} ) \geq f_1( \vect x ) - \mu n^2$, therefore:
% \begin{equation}
%       \| \mathcal N_{f_1}( \mu, \vect x ) - \vect y \|^2 \leq \| \vect x - \vect y \|^2 - 2\mu\bigl( f_1( \vect x ) - f_1( \vect y )\bigr) + 5\mu^2n^2,
% \end{equation}
From where we see that Property~\ref{prop:propopt1} is satisfied with $\rho_1( \mu, k ) = 3\mu n$. Furthermore, since for every $\vect x$ we have $\|\tilde\nabla f_{\text{Haar}}( \vect x )\| \leq \sqrt n$, formulation~\eqref{eq:HSTasSubgrad} of $\mathcal O_{f_1}$ implies that this operator satisfies Property~\ref{prop:propoptbound} with $\gamma = \sqrt n$.

It is worth remarking that the soft-thresholding is an example of a proximal operator,
\begin{equation}
   \mathcal N_{f_{\text{Haar}}}( \mu, \vect x ) = \argmin_{\vect y \in \mathbb R^n}\left\{ \mu\| H \vect y \|_ 1 + \frac12\| \vect x - \vect y \|^2 \right\}.
\end{equation}
In fact, it is possible to carry out an argumentation similar to the one that lead to inequality~\eqref{eq:propOptHaarSoftThres} above for more general proximal operators, because they too can be interpreted as examples of implicit subgradient algorithms or, alternatively, as appropriately controlled $\epsilon$-subgradient methods~\cite{col93}.

\subsubsection{Total Variation}

Another function we have used to select among the inner problem optimizers is the Total Variation~\cite{rof92}:
\begin{equation}
   f_{\text{\textsc{tv}}}( \vect x ) := \sum_{i = 1}^{\sqrt n}\sum_{j = 1}^{\sqrt n}\sqrt{( x_{i, j} - x_{i - 1, j} )^2 + ( x_{i, j} - x_{i, j - 1} )^2},
\end{equation}
where we have assumed that $n$ is a perfect square, which is true for our reconstructed images, the lexicographical notation:
\begin{equation}
   x_{i,j} := x_{i + ( j - 1 )\sqrt n}, \quad (i, j) \in \{ 1, 2, \dots, \sqrt{n} \}^2
\end{equation}
and also the following boundary conditions:
\begin{equation}
   x_{0, j} = x_{m, j}, \quad x_{i, 0} = x_{i, n}, \quad (i, j) \in \{ 1, 2, \dots, \sqrt{n} \}^2.
\end{equation}

\begin{lemma}
   Suppose $\mathcal O_f$
\end{lemma}

\subsection{Experimental Results}

\subsection{Differentiable Inner Objective Function}

In the present Subsection, we report the results obtained using Algorithm~\ref{algo:fiba} in order to approximately solve the optimization problem
\begin{equation}\label{eq:bilevelDiffInner}
   \begin{split}
      \min & \quad f_1( \vect x )\\
      \st  & \quad \vect x\in \argmin_{\vect y \in \mathbb R_+^n} \| R\vect y - \vect b \|^2\text,
   \end{split}
\end{equation}
with both $f_1( \vect x ) = \| H \vect x \|_1$ and $f_1( \vect x ) = TV( \vect x )$. Below we describe the parameter selection and explain the rationale supporting each choice.

The bilevel algorithms were compared against the Fast Iterative Soft-Thresholding Algorithm (\textsc{fista})~\cite{bet09} for the function
\begin{equation}
   \| R\vect x - \vect b \|^2 + \iota_{\mathbb R_+^n}( \vect x ),
\end{equation}
where $\iota$ is the indicator function~\eqref{eq:iota}. We have used the starting image described in the next paragraph. We iterated \textsc{fista} with a constant stepsize $\lambda = 3$, for the reasons explained in the paragraph following the next.

\paragraph{Starting image} The initial guess $\vect x_0$ used in all the experiments, for all algorithms tested, was a constant image such that $\sum_{i = 1}^m ( R\vect x_0 )_i = \sum_{i = 1}^m b_i$. It is easy to compute the correct constant value $\alpha$ from $\alpha = \sum_{i = 1}^m b_i / \sum_{i = 1}^m ( R\vect 1 )_i$ where $\vect 1$ is the vector, of appropriate dimension, with every coordinate equal to $1$. This choice makes sure that the Radon consistency condition $\sum_{i = 1}^m ( R\vect x )_i = \sum_{i = 1}^m b_i$ is satisfied for the first iteration, potentially avoiding large oscillations in the first steps of the algorithm.

\paragraph{Stepsize sequences} The sequence $\{\lambda_k\}$ was set to be
\begin{equation}\label{eq:lambdaDiff}
   \lambda_k = \frac{\lambda}{(k + 1)^{0.1}},
\end{equation}
where $\lambda_0$ was chosen to be just small enough so that the squared residual of the first iterations of the one-level algorithm is decreasing. In the examples, $\lambda_0 = 3$ worked well. This choice for $\lambda_0$ was noticed to provide the fastest inner objective function decrease during the iterations when using stepsize sequences of the form \eqref{eq:lambdaDiff} above. Sequence $\{ \eta_k \}$ was given by
\begin{equation}\label{eq:etaDiff}
   \eta_k = \frac{10^6}{( k + 1 )^{0.1}},
\end{equation}
which was chosen to attain very high values in order not to negatively influence convergence speed by limiting the values of $\lambda_{i_k}$ or $\xi_k$ (both of which remained constant throughout the iterations of Algorithm~\ref{algo:fiba}, without detected need for decreasing). Finally, the stepsize sequence $\{ \mu_k \}$ was given by
\begin{equation}\label{eq:muDiff}
   \mu_k = \frac{\mu}{k + 1}.
\end{equation}
Now, the initial stepsize $\mu_0$ has been selected in order to make the first pair of subiterations to have a specific relative strength. The precise procedure was the following: we first computed $\vect x_{1 / 3}$ as usual, following Algorithm~\ref{algo:fiba} and using the already chosen $\lambda_0$. Then, a tentative subiteration $\tilde{\vect x}_{2 / 3}$ is computed using a tentative stepsize $\tilde{\mu}_0 = 1$. Finally, the value to be used as starting stepsize is computed by
\begin{equation}\label{eq:mu0Smooth}
   \mu_0 = 10^{-2} \frac{\|\vect x_{0} - \vect x_{1 / 3}\|}{\|\vect x_{1 / 3} - \tilde{\vect x}_{2 / 3}\|}.
\end{equation}
So, the step given by the first subiteration for the inner problem is about $10^2$ times the step given by the subiteration for the outer optimization problem. This value provided a good compromise between inner problem convergence and outer function value during the iterations.

\paragraph{Algorithm Convergence} Because all entries of the matrix $R$ are nonnegative and because every pixel of the reconstructed image is crossed by several rays during acquisition, the model has the property that $X_1$ is bounded. Therefore, given the subgradient boundedness of all involved objective functions and the fact that both outer objective functions $f_{\text{Haar}}$ and $f_{TV}$ are bounded from below, Theorem~\ref{theo:convFIBA} could be applied to show that Algorithm~\ref{algo:fiba} converges in the cases covered in the present subsection, except for two issues. The first problem is that $\lambda_0$ may not be smaller than $1/L_0$, but we have observed during algorithm evaluation that the alternative sufficient decrease criterion~\eqref{eq:upperBoundLips} was satisfied in every iteration, which suffices, instead, for convergence. Furthermore, boundedness of the iterates was also observed, ensuring convergent behavior without forceful truncation.

\paragraph{Numerical Results} Figures~\ref{fig:phasePlaneDiffProb} shows that, as expected, the bilevel approach influences the iterates of the method, thereby resulting in lower outer objective function value throughout the iterations. Figure~\ref{fig:iterEvolutionDiffProb}, on the other hand and also unsurprisingly, shows that the convergence speed for the inner optimization problem is reduced as the outer optimization step influences the iterations. Figure~\ref{fig:eggImages} displays some resulting images, all with the same prescribed inner objective function value, from the algorithms and Figure~\ref{fig:eggProfiles} brings a plot of the profiles across the same line of each image.

We can see the benefits of the enforced smoothing, in particular the good quality of the Total Variation image. The advantage of the bilevel technique here is that the regularization level is chosen by a stopping criterion instead of a parameter in an optimization problem. This latter situation implies that more computational effort would be required since reconstruction for each tentative parameter value would require the equivalent to a large fraction of the computation effort of performing some iterations of the bilevel techniques.

\begin{figure}
   \input{egg_rec_axisdata.tex}%
   \centering%
   \setlength{\grftotalwidth}{\textwidth}%
   \begin{grfgraphic}[0.3]{%
      \grfxaxis{\fAxfBxaxisValues}{\fAxfBxaxisLabels}%
      \grfyaxis{\fAxfByaxisValues}{\fAxfByaxisLabels}%
      \grfxlabel{\scriptsize$\| R\vect x -  \vect b \|^2$}%
      \grfylabel[L]{\scriptsize$\| H\vect x \|_1$}%
   }%
      \grfxgrid[grfaxisstyle,gray,dotted]{\fAxfBxaxisValues}{\fAxfBxaxisValues}%
      \grfygrid[grfaxisstyle,gray,dotted]{\fAxfByaxisValues}{\fAxfByaxisValues}%
      \draw[red] plot file {egg_fistap_f0xf1.tpl};%
      \draw[green] plot file {egg_bilevel_f0xf1.tpl};%
      \draw[blue] plot file {egg_bilevel_tv_f0xf1.tpl};%
      \draw[grfaxisstyle] (\targetA,0.0) -- (\targetA,1.0);
      {%
         \tiny%
         \grftablegend[bl,fill=white]{|cl|}{%
               \hline%
               \grflegsymbol[2em]{\grflegline[red]} & \textsc{fipa}\\
               \grflegsymbol[2em]{\grflegline[green]} & \textsc{bfipsta}\\
               \grflegsymbol[2em]{\grflegline[blue]} & \textsc{bfiptva}\\
               \hline%
         }%
      }%
   \end{grfgraphic}\\%
   \input{egg_rec_tv_axisdata.tex}%
   \begin{grfgraphic}[0.3]{%
      \grfxaxis{\fAxTVxaxisValues}{\fAxTVxaxisLabels}%
      \grfyaxis{\fAxTVyaxisValues}{\fAxTVyaxisLabels}%
      \grfxlabel{\scriptsize$\| R\vect x -  \vect b \|^2$}%
      \grfylabel[L]{\scriptsize$TV( \vect x )$}%
   }%
      \grfxgrid[grfaxisstyle,gray,dotted]{\fAxTVxaxisValues}{\fAxTVxaxisValues}%
      \grfygrid[grfaxisstyle,gray,dotted]{\fAxTVyaxisValues}{\fAxTVyaxisValues}%
      \draw[red] plot file {egg_fistap_f0xTV.tpl};%
      \draw[green] plot file {egg_bilevel_haar_f0xTV.tpl};%
      \draw[blue] plot file {egg_bilevel_f0xTV.tpl};%
      \draw[grfaxisstyle] (\targetA,0.0) -- (\targetA,1.0);
      {%
         \tiny%
         \grftablegend[bl,fill=white]{|cl|}{%
               \hline%
               \grflegsymbol[2em]{\grflegline[red]} & \textsc{fipa}\\
               \grflegsymbol[2em]{\grflegline[green]} & \textsc{bfipsta}\\
               \grflegsymbol[2em]{\grflegline[blue]} & \textsc{bfiptva}\\
               \hline%
         }%
      }%
   \end{grfgraphic}%
   \caption{Logarithmic-scale plots of the trajectories followed by the three studied algorithms over the ``phase-plane'' described by $f_0 \times f_1$. The solid vertical line depicts the residual value of the images shown at Figure~\ref{fig:eggImages}. In both graphics, horizontal scale is $\| R\vect x - \vect b \|^2$. On top, vertical axis depicts $\| H\vect x \|_1$. On bottom, curve height is proportional to $ TV( \vect x )$.}%
   \label{fig:phasePlaneDiffProb}%
\end{figure}

\begin{figure}
   \input{egg_rec_iter_by_f0_axisdata.tex}%
   \centering%
   \setlength{\grftotalwidth}{\textwidth}%
   \begin{grfgraphic}[0.3]{%
      \grfxaxis{\iterxfAxaxisValues}{\iterxfAxaxisLabels}%
      \grfyaxis{\iterxfAyaxisValues}{\iterxfAyaxisLabels}%
      \grfylabel[L]{\scriptsize$\| R\vect x_k -  \vect b \|^2$}%
      \grfxlabel{\scriptsize$k$}%
   }%
      \grfxgrid[grfaxisstyle,gray,dotted]{\iterxfAxaxisValues}{\iterxfAxaxisValues}%
      \grfygrid[grfaxisstyle,gray,dotted]{\iterxfAyaxisValues}{\iterxfAyaxisValues}%
      \draw[red] plot file {egg_fistap_iterxf0.tpl};%
      \draw[green] plot file {egg_bilevel_haar_iterxf0.tpl};%
      \draw[blue] plot file {egg_bilevel_tv_iterxf0.tpl};%
      \draw[grfaxisstyle] (0.0,\targetA) -- (1.0,\targetA);
      {%
         \tiny%
         \grftablegend[tr,fill=white]{|cl|}{%
               \hline%
               \grflegsymbol[2em]{\grflegline[red]} & \textsc{fipa}\\
               \grflegsymbol[2em]{\grflegline[green]} & \textsc{bfipsta}\\
               \grflegsymbol[2em]{\grflegline[blue]} & \textsc{bfiptva}\\
               \hline%
         }%
      }%
   \end{grfgraphic}%
   \caption{Evolution of inner objective function over iterations. Solid horizontal line: residual value of the images shown in Figure~\ref{fig:eggImages}.}%
   \label{fig:iterEvolutionDiffProb}%
\end{figure}

\begin{figure}
   \input{egg_rec_axisdata.tex}%
   \centering%
   \setlength{\grftotalwidth}{\textwidth}%
   \begin{grfgraphic}{%
      \def\grfxmin{-1.115}\def\grfxmax{2.0}%
      \def\grfymin{-1.5}\def\grfymax{0.605}%
   }%
      % Vertical labels:
      \node[anchor=south,rotate=90,inner sep=\grflabelsep] at (-1.0,0.0) {\scriptsize$2048\times2048$};%
      \node[anchor=south,rotate=90,inner sep=\grflabelsep] at (-1.0,-1.0) {\scriptsize$512\times512$};%
      % Hoirizontal labels:
      \node[anchor=south,inner sep=\grflabelsep] at (-0.5,0.5) {\scriptsize\textsc{fipa}};%
      \node[anchor=south,inner sep=\grflabelsep] at (0.5,0.5) {\scriptsize\textsc{bfipsta}};%
      \node[anchor=south,inner sep=\grflabelsep] at (1.5,0.5) {\scriptsize\textsc{bfiptva}};%
%       \node[anchor=south,inner sep=\grflabelsep] at (-1.0,-1.0) {\scriptsize$512\times512$};%
      % Images:
      \node[inner sep=0pt] at (-0.5,0.0) {\includegraphics[width=\grfxunit]{egg_fistap_interpA}};%
      \node[inner sep=0pt] at ( 0.5,0.0) {\includegraphics[width=\grfxunit]{egg_bilevel_interpA}};%
      \node[inner sep=0pt] at ( 1.5,0.0) {\includegraphics[width=\grfxunit]{egg_bilevel_tv_interpA}};%
      % Profile positions:
      \draw[grfaxisstyle,red] (-1.0,\eggHprofilePos) -- (0.0,\eggHprofilePos);%
      \draw[grfaxisstyle,green] (0.0,\eggHprofilePos) -- (1.0,\eggHprofilePos);%
      \draw[grfaxisstyle,blue] (1.0,\eggHprofilePos) -- (2.0,\eggHprofilePos);%
      % Image frames:
      \draw[grfaxisstyle] (-1.0,-0.5) rectangle (0.0,0.5);%
      \draw[grfaxisstyle] (1.0,-0.5) rectangle (0.0,0.5);%
      \draw[grfaxisstyle] (1.0,-0.5) rectangle (2.0,0.5);%
      % Inset images:
      \node[inner sep=0pt] at (-0.5,-1.0) {\includegraphics[width=\grfxunit]{egg_fistap_interpA_inset}};%
      \node[inner sep=0pt] at ( 0.5,-1.0) {\includegraphics[width=\grfxunit]{egg_bilevel_interpA_inset}};%
      \node[inner sep=0pt] at ( 1.5,-1.0) {\includegraphics[width=\grfxunit]{egg_bilevel_tv_interpA_inset}};%
      % Inset squares in main images:
      \draw[grfaxisstyle] (-1.0,-1.5) rectangle (0.0,-0.5);%
      \draw[grfaxisstyle] (1.0,-1.5) rectangle (0.0,-0.5);%
      \draw[grfaxisstyle] (1.0,-1.5) rectangle (2.0,-0.5);%
      % Inset frames:
      \draw[grfaxisstyle] (\eggInsetTLX,\eggInsetTLY) rectangle (\eggInsetBRX,\eggInsetBRY);
      \draw[grfaxisstyle,shift={(1,0)}] (\eggInsetTLX,\eggInsetTLY) rectangle (\eggInsetBRX,\eggInsetBRY);
      \draw[grfaxisstyle,shift={(-1,0)}] (\eggInsetTLX,\eggInsetTLY) rectangle (\eggInsetBRX,\eggInsetBRY);
   \end{grfgraphic}%
   \caption{Reconstructions of fish egg slice from synchrotron radiation transmission data. Top-row: full slice image. Bottom row: details, with location in respective images above shown as a solid black square. The colored solid lines in the top images show the position of the profiles detailed at figure~\ref{fig:eggProfiles}.}\label{fig:eggImages}%
\end{figure}

\begin{figure}
   \input{egg_rec_axisdata.tex}%
   \centering%
   \setlength{\grftotalwidth}{\textwidth}%
   \begin{grfgraphic*}[1.0]{%
      \grfxaxis{\profAxaxisValues}{\profAxaxisLabels}%
      \grfyaxis{\profAyaxisValues}{\profAyaxisLabels}%
      \grfxlabel{\scriptsize$x_1$}%
      \grfylabel[L]{\scriptsize$\mu( x_1, \profApos )$}%
      \def\grfxmin{0.0}\def\grfxmax{1.0}%
   }%
      \grfxgrid[grfaxisstyle,gray,dotted]{\profAxaxisValues}{\profAxaxisValues}%
      \grfygrid[grfaxisstyle,gray,dotted]{\profAyaxisValues}{\profAyaxisValues}%
      \draw[red] plot file {egg_fipa_profileA.tpl};%
      \draw[green] plot file {egg_bilevel_profileA.tpl};%
      \draw[blue] plot file {egg_bilevel_tv_profileA.tpl};%
      {%
         \tiny%
         \grftablegend[tl,fill=white]{|cl|}{%
               \hline%
               \grflegsymbol[2em]{\grflegline[red]} & \textsc{fipa}\\
               \grflegsymbol[2em]{\grflegline[green]} & \textsc{bfipsta}\\
               \grflegsymbol[2em]{\grflegline[blue]} & \textsc{bfiptva}\\
               \hline%
         }%
      }%
   \end{grfgraphic*}%
   \caption{Profiles through the lines indicated in Figure~\ref{fig:eggImages}. It is noticeable the noise suppression characteristics of the Total Variation functional, while retaining image detail.}\label{fig:eggProfiles}%
\end{figure}

\subsection{Non-Differentiable Inner Objective Function}

Now we consider using Algorithm~\ref{algo:iiba} applied to optimization problem
\begin{equation}\label{eq:bilevelNonDiffInner}
   \begin{split}
      \min & \quad f_1( \vect x )\\
      \st  & \quad \vect x\in \argmin_{\vect y \in \mathbb R_+^n} \| R\vect y - \vect b \|_1\text,
   \end{split}
\end{equation}
with $f_1( \vect x ) = TV( \vect x )$. We do not experiment using $f_1( \vect x ) = \| H \vect x \|_1$ because of the visually poor reconstruction and similar optimization results, when compared to the Total Variation case, observed in the previous model.

Reconstructions were performed using algorithms where the data was divided in $s$ subsets with $s \in \{1, 2, 4, 8, 16, 32\}$. Each subset was itself composed by data comprising several projection measurements in sequence, i.e., each subset was a vertical stripe of the image\footnote{Coincidently, the vertical colored lines delimit the subsets for the case $s = 4$.} shown in the bottom of Figure~\ref{fig:experimental_Radon}. At each iteration, the sequence of subset processing was selected by a pseudo-random shuffling. This makes the algorithm non-deterministic, but still covered by the theory because every subset was used once in every iteration and each of the corresponding subdifferentials is uniformly bounded. Furthermore, we have observed a consistent behavior among runs.

The various incremental bilevel algorithms were pairwise compared against their pure projected incremental subgradient counterparts, i.e., a variation of Algorithm~\ref{algo:iiba} with $\mu_k \equiv 0$. All of the methods where started with an uniform image as described for the differentiable model. We will denote the bilevel algorithms by \textsc{iiba-}$s$, where $s$ is the number of subsets, and the projected incremental method by \textsc{inc-}$s$.

\paragraph{Stepsize sequences} The sequence $\{\lambda_k\}$ for the incremental algorithms with $s$ subsets was set to be
\begin{equation}\label{eq:lambdaNonDiff}
   \lambda_k = \frac{\lambda}{(k + 1)^{\epsilon_s}},
\end{equation}
where $\lambda$ was of the form
\begin{equation}
   \lambda = \alpha_s \frac{sf_0( \vect x_0  )}{\|\tilde \nabla f_0( \vect x_0 )\|^2},
\end{equation}
and $\tilde \nabla f_0( \vect x_0 ) \in \partial f( \vect x_0 )$. The pair $( \alpha_s, \epsilon_s )$ was selected through a simple search procedure as follows. Let us denote by $\vect x_{( s, \alpha, \epsilon )}$ the first iteration to be completed past $4$ seconds of computation time by the pure projected incremental algorithm with $s$ subsets (that is, by \textsc{inc}-$s$) and using parameters $( \alpha, \epsilon )$. Then $( \alpha_s, \epsilon_s )$ was given by
\begin{equation}
   ( \alpha_s, \epsilon_s ) := \argmin_{ (\alpha, \epsilon ) \in \{ 0.1, 0.2, \dots, 1.0 \} \times \{ 0.5, 0.6, \dots, 0.9 \} } f_0( \vect x_{( s, \alpha, \epsilon )} ).
\end{equation}
The parameters were only optimized for the non-bilevel case, and the same values were used for the corresponding (with relation to the number of subsets) bilevel algorithm. The second step sequence $\{\mu_k\}$ was prescribed as
\begin{equation}
   \mu_k = \frac{\mu}{( k + 1 )^{\epsilon_s + 0.1}},
\end{equation}
with
\begin{equation}\label{eq:mu0NonSmooth}
   \mu = 10^{-1} \frac{\|\vect x_{0} - \vect x_{1 / 3}\|}{\|\vect x_{1 / 3} - \tilde{\vect x}_{2 / 3}\|},
\end{equation}
where the rationale is the same than in~\eqref{eq:mu0Smooth}, but with target relative importance between the first subiterations of $10$.

\paragraph{Algorithm Convergence} Notice that the stepsizes are of the form
\begin{equation}
   \lambda_k = \frac{\lambda}{( k + 1 )^\epsilon}\quad\text{and}\quad \mu_k = \frac{\mu}{( k + 1 )^{\epsilon + 0.1}},
\end{equation}
where $\epsilon \in [0.5, 0.9]$ and $\lambda$ and $\mu$ are nonnegative. It is routine to check that for this range of $\epsilon$ there holds:
\begin{equation}
   \sum_{k = 0}^\infty \lambda_k = \sum_{k = 0}^\infty \mu_k = \infty, \quad \frac{\mu_k}{\lambda_k} \to 0\quad\text{and}\quad \frac{\lambda_k^2}{\mu_k} \to 0.
\end{equation}
Also, for the same reasons as in the differentiable inner problem case, the model has the property that $X_1$ is bounded. Given the subgradient boundedness of all involved objective functions and the fact that outer objective function $f_{TV}$ is bounded from below, Theorem~\ref{theo:convIIBA} can be applied to prove algorithm convergence.

\begin{figure}
   \input{inc_times.tex}%
   \centering%
   \setlength{\grftotalwidth}{\textwidth}%
   \begin{grfgraphic*}[0.3]{%
      \grfxaxis{\xaxisValues}{\xaxisLabels}%
      \grfyaxis{\yaxisValues}{\yaxisLabels}%
      \grfxlabel{\scriptsize Time ($s$)}%
      \grfylabel[L]{\scriptsize$\| R \vect x - \vect b \|_1$}%
   }%
      \grfxgrid[grfaxisstyle,gray,dotted]{\xaxisValues}{\xaxisValues}%
      \grfygrid[grfaxisstyle,gray,dotted]{\yaxisValues}{\yaxisValues}%
      \draw[red] plot file {inc_times_0.data};%
      \draw[green] plot file {inc_times_2.data};%
      \draw[blue] plot file {inc_times_4.data};%
      \draw[black] plot file {inc_times_6.data};%
      \draw[cyan] plot file {inc_times_8.data};%
      \draw[yellow] plot file {inc_times_10.data};%
      \draw[red,dashed] plot file {inc_times_1.data};%
      \draw[green,dashed] plot file {inc_times_3.data};%
      \draw[blue,dashed] plot file {inc_times_5.data};%
      \draw[black,dashed] plot file {inc_times_7.data};%
      \draw[cyan,dashed] plot file {inc_times_9.data};%
      \draw[yellow,dashed] plot file {inc_times_11.data};%
      {%
         \tiny%
         \grftablegend[tr,fill=white]{|clcl|}{%
               \hline%
               \grflegsymbol[2em]{\grflegline[red]} & \textsc{inc}-1 & \grflegsymbol[2em]{\grflegline[red,dashed]} & \textsc{inc-tv}-1\\
               \grflegsymbol[2em]{\grflegline[green]} & \textsc{inc}-2 & \grflegsymbol[2em]{\grflegline[green,dashed]} & \textsc{inc-tv}-2\\
               \grflegsymbol[2em]{\grflegline[blue]} & \textsc{inc}-4 & \grflegsymbol[2em]{\grflegline[blue,dashed]} & \textsc{inc-tv}-4\\
               \grflegsymbol[2em]{\grflegline[black]} & \textsc{inc}-8 & \grflegsymbol[2em]{\grflegline[black,dashed]} & \textsc{inc-tv}-8\\
               \grflegsymbol[2em]{\grflegline[cyan]} & \textsc{inc}-16 & \grflegsymbol[2em]{\grflegline[cyan,dashed]} & \textsc{inc-tv}-16\\
               \grflegsymbol[2em]{\grflegline[yellow]} & \textsc{inc}-32 & \grflegsymbol[2em]{\grflegline[yellow,dashed]} & \textsc{inc-tv}-32\\
               \hline%
         }%
      }%
   \end{grfgraphic*}%\\%
%    \caption{Convergence over time.}%
% \end{figure}
% \begin{figure}
%    \input{inc_iterations.tex}%
%    \centering%
%    \setlength{\grftotalwidth}{\textwidth}%
%    \begin{grfgraphic*}[0.3]{%
%       \grfxaxis{\xaxisValues}{\xaxisLabels}%
%       \grfyaxis{\yaxisValues}{\yaxisLabels}%
%       \grfxlabel{\scriptsize Iteration}%
%       \grfylabel[L]{\scriptsize$\| R \vect x - \vect b \|_1$}%
%    }%
%       \grfxgrid[grfaxisstyle,gray,dotted]{\xaxisValues}{\xaxisValues}%
%       \grfygrid[grfaxisstyle,gray,dotted]{\yaxisValues}{\yaxisValues}%
%       \draw[red] plot file {inc_iterations_0.data};%
%       \draw[green] plot file {inc_iterations_2.data};%
%       \draw[blue] plot file {inc_iterations_4.data};%
%       \draw[black] plot file {inc_iterations_6.data};%
%       \draw[cyan] plot file {inc_iterations_8.data};%
%       \draw[yellow] plot file {inc_iterations_10.data};%
%       \draw[red,dashed] plot file {inc_iterations_1.data};%
%       \draw[green,dashed] plot file {inc_iterations_3.data};%
%       \draw[blue,dashed] plot file {inc_iterations_5.data};%
%       \draw[black,dashed] plot file {inc_iterations_7.data};%
%       \draw[cyan,dashed] plot file {inc_iterations_9.data};%
%       \draw[yellow,dashed] plot file {inc_iterations_11.data};%
%       {%
%          \tiny%
%          \grftablegend[tr,fill=white]{|clcl|}{%
%                \hline%
%                \grflegsymbol[2em]{\grflegline[red]} & \textsc{inc}-1 & \grflegsymbol[2em]{\grflegline[red,dashed]} & \textsc{inc-tv}-1\\
%                \grflegsymbol[2em]{\grflegline[green]} & \textsc{inc}-2 & \grflegsymbol[2em]{\grflegline[green,dashed]} & \textsc{inc-tv}-2\\
%                \grflegsymbol[2em]{\grflegline[blue]} & \textsc{inc}-4 & \grflegsymbol[2em]{\grflegline[blue,dashed]} & \textsc{inc-tv}-4\\
%                \grflegsymbol[2em]{\grflegline[black]} & \textsc{inc}-8 & \grflegsymbol[2em]{\grflegline[black,dashed]} & \textsc{inc-tv}-8\\
%                \grflegsymbol[2em]{\grflegline[cyan]} & \textsc{inc}-16 & \grflegsymbol[2em]{\grflegline[cyan,dashed]} & \textsc{inc-tv}-16\\
%                \grflegsymbol[2em]{\grflegline[yellow]} & \textsc{inc}-32 & \grflegsymbol[2em]{\grflegline[yellow,dashed]} & \textsc{inc-tv}-32\\
%                \hline%
%          }%
%       }%
%    \end{grfgraphic*}%
   \caption{Convergence of incremental and incremental bilevel algorithms: inner objective function value as a function of computation time.}\label{fig:nonDiffIncrConvTime}%
\end{figure}

\begin{figure}
   \input{inc_tv_res.tex}%
   \centering%
   \setlength{\grftotalwidth}{\textwidth}%
   \begin{grfgraphic*}[0.3]{%
      \grfxaxis{\xaxisValues}{\xaxisLabels}%
      \grfyaxis{\yaxisValues}{\yaxisLabels}%
      \grfxlabel{\scriptsize $\| R \vect x - \vect b \|_1$}%
      \grfylabel[L]{\scriptsize $TV( \vect x )$}%
      \def\grfymax{1.3}%
   }%
      {%
         \def\grfymax{1}%
         \grfxgrid[grfaxisstyle,gray,dotted]{\xaxisValues}{\xaxisValues}%
         \grfygrid[grfaxisstyle,gray,dotted]{\yaxisValues}{\yaxisValues}%
      }%
      \draw[red] plot file {inc_tv_res_0.data};%
      \draw[green] plot file {inc_tv_res_2.data};%
      \draw[blue] plot file {inc_tv_res_4.data};%
      \draw[black] plot file {inc_tv_res_6.data};%
      \draw[cyan] plot file {inc_tv_res_8.data};%
      \draw[yellow] plot file {inc_tv_res_10.data};%
      \draw[red,dashed] plot file {inc_tv_res_1.data};%
      \draw[green,dashed] plot file {inc_tv_res_3.data};%
      \draw[blue,dashed] plot file {inc_tv_res_5.data};%
      \draw[black,dashed] plot file {inc_tv_res_7.data};%
      \draw[cyan,dashed] plot file {inc_tv_res_9.data};%
      \draw[yellow,dashed] plot file {inc_tv_res_11.data};%
      {%
         \tiny%
         \grftablegend[tr,fill=white]{|clcl|}{%
               \hline%
               \grflegsymbol[2em]{\grflegline[red]} & \textsc{inc}-1 & \grflegsymbol[2em]{\grflegline[red,dashed]} & \textsc{inc-tv}-1\\
               \grflegsymbol[2em]{\grflegline[green]} & \textsc{inc}-2 & \grflegsymbol[2em]{\grflegline[green,dashed]} & \textsc{inc-tv}-2\\
               \grflegsymbol[2em]{\grflegline[blue]} & \textsc{inc}-4 & \grflegsymbol[2em]{\grflegline[blue,dashed]} & \textsc{inc-tv}-4\\
               \grflegsymbol[2em]{\grflegline[black]} & \textsc{inc}-8 & \grflegsymbol[2em]{\grflegline[black,dashed]} & \textsc{inc-tv}-8\\
               \grflegsymbol[2em]{\grflegline[cyan]} & \textsc{inc}-16 & \grflegsymbol[2em]{\grflegline[cyan,dashed]} & \textsc{inc-tv}-16\\
               \grflegsymbol[2em]{\grflegline[yellow]} & \textsc{inc}-32 & \grflegsymbol[2em]{\grflegline[yellow,dashed]} & \textsc{inc-tv}-32\\
               \hline%
         }%
      }%
   \end{grfgraphic*}%
   \caption{Total variation versus residual norm-1. This graphics are example of a very specific experimental setup for the optimization algorithm, where the secondary objective function is monotonically dependent, at a given 1-norm residual, on the incrementality level.}\label{fig:nonDiffPhasePlane}%
\end{figure}

\paragraph{Numerical Results} By denoting $R_i$, $i \in \{1, 2, \dots, s\}$, the matrix with the rows corresponding to the $i$-th subset, we notice that the computationally demanding parts of the algorithm are products of the form
\begin{equation}
   R_i\vect x\quad\text{and}\quad R_ i^T\vect y,
\end{equation}
because the partial subgradients are given by
\begin{equation}
   R_ i^T\vect{\sign}(R_i \vect x - \vect b).
\end{equation}
We were not able to make the \textsc{nfft} library as efficient for such partial matrix-vector products, which imposed a large overhead in the partial iterations. We have instead used a ray-tracing algorithm~\cite{hly99,sid85} implemented to run in \textsc{gpu}s (Graphics Processing Units) under single precision floating point arithmetics.

A special scheme was used so that access to slow \textsc{gpu} memory is minimized by performing the computations in sub-images loaded to/from the \textsc{gpu}'s shared memory (a $64$kb fast L1-cache-like memory) in coalesced reads/writes, and summing up the partial results. In this setting, the sequential computation of the $s$ different partial subgradients takes longer than the computation of the subgradient itself, because there are more memory copy to/from shared memory. Yet another per-iteration overhead of the incremental methods are the multiple subiteration updates. Therefore one iteration of the incremental method with $s$ subsets still takes slightly longer than with $s - 1$ subsets.

Even with mandatory overheads, a careful implementation was able to make the iteration-wise speed up provided by the incremental approach advantageous time-wise, as can be seen in Figure~\ref{fig:nonDiffIncrConvTime}. An important feature in this plot is that this speed up is retained by the bilevel algorithms in a similar fashion to the non-bilevel incremental method. That is, if we take into account that considering the secondary objective function in the optimization does, expectedly, slow down the non-incremental method from the viewpoint of primary objective function decrease, it can be seen that incremental bilevel techniques too present a speed up in this convergence rate as the number of subsets grow.

A particular point in the experimental results can be seen in Figure~\ref{fig:nonDiffPhasePlane}. In the application of tomographic reconstruction, incrementalism seems to induce more roughness and we therefore see that \textsc{inc}-$s$ achieves lower Total Variation for the same value of 1-norm of the residual than \textsc{inc}-$2s$. Looking at the \textsc{iiba}-$s$ curves in the same plot, we notice that the choice of secondary objective function, which is conflicting with the incrementality idea, also plays a similar role in the bilevel case. Consequently, at least for our algorithmic parameters selection, there is a incrementality level (or equivalently, primary objective function decrease speed) versus secondary objective function decrease trade-off. Even so, \textsc{iiba}-$32$ provides substantially lower Total Variation for a given 1-norm of the residual compared to \textsc{inc}-$s$ for every $s$ while still achieving faster experimental primary objective function decrease rate than \textsc{inc}-$s$ with $s \leq 4$.

For other bilevel models, at first glance, there seems not to be any reason for an increase in incrementality to lead to worse secondary to primary objective function ratios. However, such antagonism between fast algorithms (with relation to data adherence) and desirable solution properties may appear naturally in ill-posed inverse problems like the one we consider here, because in this case overly fit solutions to noisy data are unstable.

\section{Conclusions}

We have presented two classes of algorithms for instances of bilevel non-differentiable convex optimization problems. The proposed algorithms have computationally simple iterations. We have numerically demonstrated that this feature allows applicability to real world problems of huge size involving tomographic image reconstruction, in this case synchrotron-light illuminated biological samples. Algorithmic flexibility was highlighted by two conceptually distinct implementations: on one side, a \textsc{nfft}-based, thus algorithmically fast, high-level implementation in the Python language, which is highly portable to most computing architectures and environments. On the other hand, the simplicity of the method was also suitable for a low-level hardware-specific implementation fully running on a \textsc{gpu} with no external software library dependency.

The presented techniques were developed with early stopped, moderately precise solutions, in mind. No stopping criterion was given, as is common for $\epsilon$-subgradient algorithms

\section*{Acknowledgements}

We would like to thank the LNLS for providing the beam time for the tomographic acquisition, obtained under proposal number 17338. We also want to thank Prof. Marcelo dos Anjos (Federal University of Amazonas) for kindly providing the fish egg samples used in the presented experimentation.

% \begin{figure}
%    \centering%
%    \setlength{\grftotalwidth}{\textwidth}%
%    \begin{grfgraphic}{%
%       \def\grfxmin{-1.0}\def\grfxmax{1.0}%
%       \def\grfymin{-0.5}\def\grfymax{0.5}%
%    }%
%       \node[inner sep=0pt] at (-0.5,0.0) {\includegraphics[width=\grfxunit]{egg_bilevel}};%
%       \node[inner sep=0pt] at ( 0.5,0.0) {\includegraphics[width=\grfxunit]{egg_fistap}};%
%       \draw[grfaxisstyle] (-1.0,-0.5) rectangle (0.0,0.5);%
%       \draw[grfaxisstyle] (1.0,-0.5) rectangle (0.0,0.5);%
%    \end{grfgraphic}%
%    \caption{Reconstructions of fish egg slice from synchrotron radiation transmission data. Left: result from bilevel approach; right: result from \textsc{fista}.}%
% \end{figure}

% We have shown convergence for our algorithm under mild
% hypothesis, except maybe the boundedness of $X$. We have to
% remark, however, that while this hypothesis seems rather
% strong, in every one of the above proofs, what was actually
% used is the consequence that both $d^g_{X_0}( \delta )$ and
% $d^f_{X_1}( \delta )$ are well defined and vanish as $\delta
% \to
% 0$. Equivalently, what our algorithmic scheme needs to work
% is that being distant from the optimal set, but still inside
% (or near) the feasible set, does imply that the value of the
% objective function increases, which is a rather realistic
% assumption. In particular, if we make the \emph{a priori}
% assumption that the iterations are bounded, then
% $\lim_{\delta \to 0}d_{X_0}^g( \delta ) = \lim_{\delta \to
% 0}d_{X_1}^f( \delta ) = 0$. Therefore, our results lead to
% the
% following:
% \begin{theorem}\label{theo:ConvBound}
%    Assume the sequence $\{ x_k \}$ generated by
% algorithm~\eqref{eq:algo} is bounded and belongs, $\mathcal
% O_f$ and $\mathcal O_{f_1}$ satisfy
% Properties~\ref{prop:propopt1}--\ref{prop:propoptbound} with
% $\{ \rho^g_k \}$ such that $\lambda_k\rho^g_k/\mu_k \to 0$
% and $\mathcal F_{X_0}$ obeys Property~\ref{prop:propfac}
% with
% $\varepsilon$ such that
% $\lambda_k^{1+\varepsilon}/\mu_k\to0$. Suppose also that
% the stepsizes satisfy $\sum_k\mu_k = \sum_k\lambda_k =
% \infty$, $\mu_k \to 0$, $\lambda_k \to 0$, and
% $\mu_k/\lambda_k \to 0$, then
%    \begin{equation*}
%       d_{X_2}( x_k ) \to 0\text.
%    \end{equation*}
% \end{theorem}
% \begin{proof}
%    First we notice that boundedness of $\{ x_k \}$ implies
% that $d_{X_1}( x_k )$ is bounded and $\lambda_k \to 0$
% together
% with~\eqref{eq:propfacforte2} imply $d_{X_0}( x_k ) \to 0$.
% Also, the boundedness assumption on $\partial g$ required
% for Lemma~\ref{lemm:CX} to hold are satisfied because $\{
% x_k \}$ is bounded. Therefore, we cannot apply
% Lemma~\ref{lemm:CX} here only because we have not assumed
% $X$ to be bounded. However, $\{ x_k \}$ being bounded
% implies $\lim_{\delta \to 0}d_{X_0}^g( \delta )=0$ and the
% proof
% of Lemma~\ref{lemm:CX} works just the same if we replace
% boundedness of $X$ by the assumption that this limit holds,
% therefore we have shown that $d_{X_1}( x_k ) \to 0$.
% 
%    Now, all assumptions for Lemma~\ref{lemm:CX*} are
% satisfied except that we don't assume boundedness of $X_2$,
% but, again, the proof for this result works exactly the same
% if the boundedness assumption on $X_2$ is replaced by
% $\lim_{\delta \to 0}d_{X_1}^f( \delta )=0$, which is a
% consequence of boundedness of $\{ x_k \}$.
% \end{proof}
% 
%  Therefore, in cases where convergence may not hold, we must necessarily have an unbounded sequence of iterates, a fact that could be detected during the execution of the algorithm. Even though unboundedness of the iterations does not necessarily mean that we are not approaching the desired optimal and stopping the algorithm under this circumstance seems to be an overreaction, it is more likely that some realistic bound on the optimal solution can be found to the problem at hand and implemented directly on the method through, say, projection onto some box or ball and then convergence is assured. So, even though boundedness of $X$ is a simplifying assumption, it is one that does not hurt. It does not hide complications in the proofs that would otherwise make the theory less understandable, neither it seems to pose major difficulties when applying the algorithm in practice.

\endinput


==> inc_iterations.tex <==
\def\xaxisLabels{[]\tiny$0.00$;\tiny$225.50$;\tiny$451.00$;\tiny$676.50$;\tiny$902.00$[]}
\def\xaxisValues{[]0.00000;0.25000;0.50000;0.75000;1.00000[]}
\def\yaxisLabels{[]\tiny$4.44\cdot 10^{3}$;\tiny$3.25\cdot 10^{4}$;\tiny$2.38\cdot 10^{5}$[]}
\def\yaxisValues{[]0.00000;0.50000;1.00000[]}


==> operators.tex <==
\section{Operators}\label{sec:operators}

This section is devoted to the construction of operators satisfying the required properties for algorithm~\eqref{eq:algo} to converge. We first consider the \emph{optimality operators} $\mathcal O_f$ and $\mathcal O_g$, mentioning classical instances based on subgradient iterations and proceeding further to incremental operators that had already appeared in~\cite{hed09}, then we exhibit a new example inspired by Bertsekas' paper~\cite{ber11} on incremental proximal methods. Finally, we move on to show how to obtain suitable \emph{feasibility operators} $\mathcal F_C$ such that the required characteristics for convergence of the iterations holds.

\subsection{Optimality Operators}

We begin by noticing that subgradient steps, under mild assumptions, satisfy Properties~\ref{prop:propopt1}--\ref{prop:propoptbound}. All that is required is that the stepsize goes to zero and that the subgradients are bounded. To see that this is true, let us denote $\mathcal S_f( \lambda, x ) := x - \lambda \tilde\nabla f( x )$, where $\tilde\nabla f( x ) \in \partial f( x )$, then, as it is well known, we have, for $\lambda \geq 0$:
\begin{equation*}
   \| \mathcal S_f( \lambda, x ) - y \|^2 \leq \| x - y \|^2 - \lambda\bigl( f( x ) - f( y ) \bigr) + \lambda^2\| \tilde\nabla f( x ) \|^2
\end{equation*}
and, obviously,
\begin{equation*}
   \| \mathcal S_f( \lambda, x ) - x \| = \lambda\| \tilde\nabla f( x ) \|\text.
\end{equation*}

Since projections obviously satisfy Property~\ref{prop:propfac} with $E = 0$ and any $\varepsilon$, we conclude, according to Theorem~\ref{theo:ConvBound}, that the following algorithm is convergent (we shall not repeatedly state technical conditions on the boundedness of $X$ or $\{ x_k \}$) if the setpsizes satisfy $\sum_k\lambda_k = \sum_k\mu_k = \infty$, $\lambda_k / \mu_k \to 0$, $\mu_k^2 / \lambda_k \to 0$, and the relevant subgradient are bounded:
\begin{equation*}
   \begin{split}
      x_{k+1/3} &{}= x_k - \lambda_k\tilde\nabla f( x_k )\text;\\
      x_{k+2/3} &{}= x_{k+1/3} - \mu_k\tilde\nabla g( x_{k+1/3} )\text;\\
      x_{k+1} &= \proj_C( x_{k+2/3} )\text.
   \end{split}
\end{equation*}
While the above algorithm is interesting on its own, more relevant when viewed from the existing literature viewpoint is the following slightly modified version of it. The following algorithm converges to the optimal set of problem~\ref{eq:bilevel}:
\begin{equation}\label{eq:SolEquiv}
   \begin{split}
      x_{k+1/3} &{}= x_k - \lambda_k\tilde\nabla f( x_k )\text;\\
      x_{k+2/3} &{}= x_{k+1/3} - \mu_k\tilde\nabla g( x_k )\text;\\
      x_{k+1} &= \proj_C( x_{k+2/3} )\text.
   \end{split}
\end{equation}
To see that this is true, we notice that we have, for this method:
\begin{equation*}
   \begin{split}
      \| x_{k+2/3} - y \|^2 &{}\leq \| x_{k+1/3} - y \|^2 - \mu_k\bigl( g( x_k ) - g( y ) \bigr) + \mu_k^2\|\tilde\nabla g( x_k )\|^2\\
         &{}= \| x_{k+1/3} - y \|^2 - \mu_k\bigl( g( x_{k+1/3} ) - g( y ) \bigr) + \mu_k^2\|\tilde\nabla g( x_k )\|^2\\
         &\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad {}+\mu_k\bigl( g( x_{k+1/3} ) - g( x_k ) \bigr)\\
         &{}\leq \| x_{k+1/3} - y \|^2 - \mu_k\bigl( g( x_{k+1/3} ) - g( y ) \bigr) + \mu_k^2\|\tilde\nabla g( x_k )\|^2\\
         &\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad {}+\mu_k\lambda_k\|\tilde\nabla g( x_{k+1/3} )\|\|\tilde\nabla f( x_k )\|\text,
   \end{split}
\end{equation*}
therefore, it essentially does not matter whether the subgradient used in the second subiteration is computed at $x_k$ or $x_{k+1/3}$.

Let $F_{\sigma}( x ) := \sigma f( x ) + g( x )$, then notice that iterations~\eqref{eq:SolEquiv} are clearly equivalent to $x_{k+1} = \proj_C\bigl( x_k + \mu_k\tilde\nabla F_{\sigma_k}( x_k ) \bigr)$, where $\sigma_k = \lambda_k / \mu_k$. This is the algorithm presented in~\cite{sol07}, except that now there is no differentiability hypothesis and that no line search has to be performed. In another approach, a bundle-like method was used to proceed in a descent direction for a non-differentiable $F_\sigma$ in~\cite{sol08}. We have here shown that there is no need to seek for a descent direction, an approximate subgradient iteration will do. To be fair, however, we must mention that the theoretical hypothesis for convergence in~\cite{sol07,sol08} require only boundedness of $X^*$, while we demand $X$ (or $\{ x_k \}$) to be bounded. On the other hand, while we have presented algorithm~\eqref{eq:SolEquiv} using $\proj_C$ as the feasibility operator, our approach is more general in that this projection is not strictly necessary, which makes our method a somewhat farther reaching generalization than merely removing the line search or the bundle minimization from the algorithms of~\cite{sol07,sol08}. Therefore, in the case where $X^*$ is known to be bounded, but $X$ is not, if a bound $\delta$ on $\| x \|$ for every $x \in X^*$ could be computed, than one could replace $C$ by $C \cap B_\delta( 0 )$ in the formulation of the problem that all boundedness assumptions would be satisfied.

We now shall briefly mention some of the incremental methods that are suitable for being used as optimality operators within our algorithms. All of them have already appeared in previous literature, we only summarize them here, in order to make clear how general our definition of the optimality operator is and to show how easy it is to apply such a definition in order to obtain incremental algorithms for the task of convex bilevel optimization.

We first notice that any of the optimality operators in~\cite{hed09} satisfy Properties~\ref{prop:propopt1}--\ref{prop:propoptbound}, since they are defined this very way. Therefore, any $\epsilon$-subgradient (including most incremental subgradient and incremental aggregated subgradient) method satisfies the required assumptions. In particular, we have the following results, which show that, as we have already mentioned, any of the iterations iterations~\eqref{eq:gradinc}--\eqref{eq:subgradagr} do fulfill Properties~\ref{prop:propopt1}--\ref{prop:propoptbound} if one replaces $X$ on the required projections by $Y\supseteq X$, where $Y$ is a superset of $X$ such that one can compute a projection onto $Y$. Here we only mention the relevant results and refer the reader to reference~\cite{hed09} for the proofs. The reader must be aware that we state the results are stated for the case where each operator is used as $\mathcal O_f$, for the $\mathcal O_g$ case, it the same results hold with the roles of $\lambda_k$ and $\mu_k$ exchanged and $f$ replaced by $g$.

\begin{proposition}
   Assume the subgradient boundedness assumption
   \begin{equation}\label{eq:sgl}
      \| v \| \leq K_l\text, \quad \forall v \in \partial f_l( x_k ) \cup \partial f_l( x_{k,l-1} )\text, \quad l = 1, \dots, m\text, \quad k = 0, 1, \dots
   \end{equation}
   Then the iterations \eqref{eq:gradinc}~and~\eqref{eq:subgradinc} satisfy Property~\ref{prop:propopt1} with  $\rho_k\leq\lambda_k(\sum_{l=1}^mK_l)^2$ and $\beta=2$, and Property~\ref{prop:propoptbound} with $\gamma=\sum_{l=1}^mK_l$.
\end{proposition}
\begin{proof}
   The first part is from~\cite[Lemma~2.1]{neb01}, while that Property~\ref{prop:propoptbound} holds can be immediately seen from the hypothesis and the definition of the operator.
\end{proof}

\begin{proposition}
   Assume that \eqref{eq:sgl} holds. Then iterations~\eqref{eq:subgradagr} satisfies Property~\ref{prop:propopt1} with $\beta=2$ and
   \begin{equation*}
      \rho_k=(4+1/m){\overline\lambda}_kK^2+4K\bigl( 2d_{C}( x_{k - 1/3} ) + \mu_{k-1}\gamma \bigr)\text,
   \end{equation*}
   where $K:=\sum_{l=1}^mK_l$ and ${\overline\lambda}_k:=\max\{\lambda_k,\lambda_{k-1}\}$ for $k>0$. It also satisfies Property~\ref{prop:propoptbound} with $\gamma=C$.
\end{proposition}
\begin{proof}
    The proof is nearly identical of the one provided for~\cite[Proposition~3.2]{hed09}, with minor changes in order to accommodate the fact that there is an extra step between two successive applications of the aggregated operator. We omit the details.
\end{proof}

Paper~\cite{hed09} already discusses the above operators, so, now we consider another one which we can add to the set of those available for our algorithm: the incremental proximal iteration. Indeed, let us consider that our objective function has the following structure:
\begin{equation*}
      \min\quad f(x) := \displaystyle\sum_{i=1}^m F_i(x)
\end{equation*}
where $F_i(x) = f_i(x)+h_i(x)$, with $f_i:\mathbb{R}^n\rightarrow \mathbb{R}$ and $h_i:\mathbb{R}^n\rightarrow \mathbb{R}$ convex functions such that $f_i$ is appropriate for a proximal iteration, while $h_i$ is more suitable for a subgradient step. Then we recall the following algorithms that are presented in \cite{ber11}:

\begin{enumerate}
   \item \label{algo:prox1}
      \begin{equation*}
         \begin{split}
            z_{k, i} &{}= \arg\min_{x\in Y}\left\{ f_i( x ) + \frac{1}{2\lambda_k}\| x - x_{k, i-1} \|^2 \right\}\text, \\
            x_{k, i} &{}= \proj_Y\left( z_k - \lambda_k\tilde\nabla h_{i}( z_{k, i} ) \right)\text;
         \end{split}
      \end{equation*}

   \item \label{algo:prox2}
      \begin{equation*}
         \begin{split}
            z_{k, i} &{}= \arg\min_{x\in \mathbb{R}^n}\left\{ f_i( x ) + \frac{1}{2\lambda_k}\| x - x_{k, i-1} \|^2 \right\}\text, \\
            x_{k, i} &{}= \proj_Y\left( z_{k, i} - \lambda_k\tilde\nabla h_{i}( z_{k, i} ) \right)\text;
         \end{split}
      \end{equation*}

   \item \label{algo:prox3}
      \begin{equation*}
         \begin{split}
            z_{k, i} &{}= x_{k, i-1} - \lambda_k\tilde\nabla h_{i}( x_{k, i-1} )\text, \\
            x_{k, i} &{}= \arg\min_{x\in Y}\left\{ f_i( x ) + \frac{1}{2\lambda_k}\| x - z_{k, i} \|^2 \right\}\text;
         \end{split}
      \end{equation*}

   \item \label{algo:prox4}
      \begin{equation*}
         x_{k, i} = \arg\min_{x\in Y}\left\{ f_i( x ) + \tilde\nabla h_i( x_{k, i-1} )^T( x - x_{k, i-1} )+\frac{1}{2\lambda_k}\| x - x_{k, i-1} \|^2 \right\}\text.
      \end{equation*}

\end{enumerate}

In each of the iterations above, $\tilde{\nabla}h_i(x)$ is some subgradient of $h_i$ at $x$, the iterations run from $i = 1$ to $i=m$ and $x_{k, 0} = x_{k}$. Consider that $\mathcal O_f( \lambda_k, x_{k} )$ is then given by $x_{k, m}$, then, \cite[Proposition~3]{ber11} immediately implies the following result:

\begin{proposition}
Suppose that the subgradients of $f_i$ and $g_i$ are bounded, then each of the Algorithms~\ref{algo:prox1}--\ref{algo:prox4}, when used as optimality operator for our method, satisfy Properties~\ref{prop:propopt1}--\ref{prop:propoptbound}.
\end{proposition}

\subsection{Feasibility Operators}\label{subsec:feaop}


This section deals with the construction of practical operators that satisfy Properties~\eqref{prop:propfac}. We first notice that if, for every $x \in C$ and any $y \notin C$, $\| \mathcal E_C( y ) - x \|^2 < \| y - x \|^2$ holds for a continuous operator $\mathcal E_C$, then any number of repeated application of this operator still respects~\eqref{eq:propfacforte1}. Furthermore, in this case iteration of $\mathcal E_C$ converges to $C$, so all we need is a Fejér-monotone operator coupled with a suitable stopping criterion. Since those operators abound (see, e.g, \cite[Subsection~3.2]{hed09} and \cite{com97}), we show how to devise such a criterion.

If we have available some function $\phi : \mathbb R^n \to \mathbb R$ such that
\begin{equation}\label{eq:cres1}
   \phi( x ) \geq Md_C^\alpha( x )
\end{equation}
for some $M > 0$ and $\alpha > 0$, it is an easy task: iterate until the point $y = \mathcal E_C^p( x_k )$ satisfies $\phi( y ) \leq K\mu^{\alpha\varepsilon}$ for some (user-specified) $K>0$. If this is so, then $d_C( y ) \leq \mu^\varepsilon K^{1/\alpha} / M$, and, therefore, the following operator will satisfy~\eqref{eq:propfacforte2} with $E = K^{1/\alpha} / M$:
\begin{equation}\label{eq:repfeaop}
   \mathcal F_C( \mu, x ) := \mathcal E_C^{p( \mu, x )}( \mu, x )\text,
\end{equation}
where
\begin{equation}\label{eq:repfeaoptest}
   p( \mu, x ) := \min\{ p \in \mathbb N : \phi\bigl( \mathcal E_C^p( x ) \bigr) \leq K\mu^{\alpha\varepsilon}\}\text.
\end{equation}
Notice that the stopping criterion is independent of $M$, which is, therefore, unnecessary in practice. We need to know $\alpha$, but in most circumstances we will find this value to be $1$, as we shall soon see.

By now we have assumed that there is a function $\phi$ such that~\eqref{eq:cres1} holds. Our next step is to provide some cases where such a function is available. Before proceeding, we provide some standard results and definitions (see \cite{hil93,ber03}) which will be useful in the development.
\begin{definition}[Normal Cone]
   We define the normal cone of $C$ at $x$ as
   \begin{equation*}
      N_C( x ) := \{ s : \langle s, y - x \rangle \leq 0\text, \quad\forall y \in C \}\text.
   \end{equation*}
\end{definition}

The normal cone is only interesting when $x$ on $\bound C$, because when that is the case, separation theorems ensure $N_C( x )$ is nonempty. This concept plays a role in our analysis because $N_C( x )$ is the set of directions $s$ such that $x + s$ will be projected at $x$, as the next Theorem indicates.

\begin{theorem}\label{teo:convex1}
   Let $C$ be an non-empty, closed and convex set. An element $p\in C$ is the projection $\proj_C( x )$ if and only if
   \begin{equation*}
      \langle x - p, y - p \rangle \leq 0\text, \quad\forall y \in C\text.
   \end{equation*}
\end{theorem}

It is sometimes possible to characterize $N_C( x )$ in terms of $\partial \phi( x )$ if $C$ is a sublevel set of $\phi$.
\begin{theorem}\label{teo:convex2}
   Let $\phi:\mathbb{R}^n \rightarrow \mathbb R$ be a convex function and suppose that $0\notin \partial \phi(x)$, then
   \begin{equation*}
      N_{\lev \phi(x) } ( x ) = \mathbb R_+\partial \phi(x)\text,
   \end{equation*}
   where $\mathbb R_+ = [ 0, \infty )$.
\end{theorem}

Armed with these results we can devise a simple condition that implies~\eqref{eq:cres1} in the case
\begin{equation}\label{eq:Csimp}
   C = \lev_0( \phi )\text.
\end{equation}
\begin{proposition}\label{prop:growsimp}
   Let $C$ be given by~\eqref{eq:Csimp} and assume that there is $V > 0$ such that for every $x$ in $\bound \lev_0( \phi )$ (that is, the boundary of $\lev_0( \phi )$) we have
   \begin{equation}\label{eq:subboundforte}
      v \in \partial \phi( x ) \Rightarrow \|v\| \geq M\text.
   \end{equation}
   Then $\phi( y ) \geq Md_C( y )$ for all $y \notin C$.
\end{proposition}
\begin{proof}
   Let $x = \proj_{\lev_0( \phi )}( y )$ and $d = y - x$. Theorem~\ref{teo:convex1} means that $d$ is in $N_C( x )$, so, because $C = \lev_0( \phi )$ and $\phi( x ) = 0$, Theorem~\ref{teo:convex2} implies that $d = tv$ for some $t > 0$ and some $v \in \partial \phi( x )$; for such a $v$ we have $d^Tv = \| d \| \| v \|$. On the other hand, $\phi( y ) \geq \phi( x ) + w^Td = w^Td$, $\forall w\in \partial \phi( x )$. In particular, for $w = v$, we have
   \begin{equation*}
      \phi( y ) \geq v^Td = \| v \| \| d \| = \| v \| d_C( y ) \geq M d_C( y )\text,
   \end{equation*}
   as desired.
\end{proof}

Proposition~\ref{prop:growsimp} is also useful when we discuss a more general setting, in which we assume the feasible set to be made of the intersection of several convex sets, each described as the sublevel set of a convex function.

Consider a set $C = \bigcap_{i=1}^r C_i$, where $C_i = \lev_0( \phi_i )$ and each $\phi_i$ is a convex function. We assume that for every $\phi_i$ there holds a growth condition like
\begin{equation}\label{eq:indgrow}
   \phi_i( x ) \geq Md_{C_i}^\alpha( x )\text, \quad \forall x \notin C_i\text,
\end{equation}
and ask ourselves when is it possible to ensure a similar relation between $\phi( x ) := \max\{ \phi_i( x ) \}$ and $d_C( x )$. To answer that question we present first a proposition that can be found in~\cite{hof92}:
\begin{proposition}\label{prop:relationdist}
   Let $X$ be an inner product space and $C_1, \dots, C_r$ convex subsets of $X$. Suppose that there exist $D > 0$ and $\rho > 0$ such that $\sup_{ x, y \in C_i} d(x,y) < D$ for all $i = 1, \dots, r$ and
   \begin{equation}\label{eq:condred}
      \rho < \sup_{x\in C}~d\left(x,X\backslash \bigcap_{i=1}^{r-1} C_i\right)\text,
   \end{equation}
   where $C = \displaystyle\bigcap_{i=1}^r C_i$. Then, if $d_{C_i}(x) \leq \epsilon$ for all $i=1,\hdots, r$, it follows that
   \begin{equation*}
      d_C( x ) \leq \frac{2\left( \frac{D-\rho}{\rho} \right)^{r+1} - \left( \frac{D-\rho}{\rho} \right)^{r} - \left( \frac{D-\rho}{\rho} \right)}{\left( \frac{D-\rho}{\rho} \right)-1}\epsilon\text.
   \end{equation*}
\end{proposition}

We remark that the requirement~\eqref{eq:condred} holds for a large class of sets, for example, when $\inte C\neq \emptyset$, as the following result shows:
\begin{proposition}\label{prop:intdist}
   Let $X$ be an inner product space and $C_1,\hdots,C_r$ convex subsets of X. Let $C = \bigcap_{i = 1}^r C_i$ and assume $\inte C \neq \emptyset$, then condition~\eqref{eq:condred} is satisfied.
\end{proposition}
\begin{proof}
   Since $C$ is defined as the intersection of the sets $C_i$, it follows immediately that
   \begin{equation*}
      C\cap\left(X\backslash\bigcap_{i=1}^{r-1} C_i\right) = \emptyset\text.
   \end{equation*}
   Therefore, because $\inte C \neq \emptyset$, we can exhibit $c\in C$ and $\sigma > 0$ such that
   \begin{equation*}
      B( c, \sigma )\cap\left(X\backslash\bigcap_{i=1}^{r-1} C_i\right) = \emptyset\text.
   \end{equation*}
   Consequently, the result follows since we have
   \begin{equation*}
      \sigma \leq \sup_{x\in C}~d\left(x,X\backslash \bigcap_{i=1}^{r-1} C_i\right)\text,
   \end{equation*}
   which ends the proof.
\end{proof}

Let us now return to the situation of~\eqref{eq:indgrow} and answer the question raised there.
\begin{proposition}
   Let $C = \bigcap_{i = 1}^r C_i$, where the $C_i$ are closed convex sets, $A\subset \mathbb{R}^n$ be a bounded closed convex, and assume that there are $\overline{M} > 0$ and $\alpha > 0$ such that
	\begin{equation}\label{majorhi}
		d_{C_i}(x)\leq \overline{M}h_i(x)^\alpha\text,\quad i=1,\hdots,r
	\end{equation}
	for some functions $h_i : \mathbb R^n \to \mathbb R$. Suppose further that there exists $\rho > 0$ such that
	\begin{equation}\label{eq:condredb}
		\rho < \sup_{x\in A\cap C}~d\left(x,\mathbb{R}^n\backslash \bigcap_{i=1}^{r-1} [A\cap C_i]\right)\text.
	\end{equation}
	Then there is $M > 0$ such that the following inequality holds for every $x \in A$:
	\begin{equation*}
		\phi( x ) \geq Md_{C}^\alpha( x )\text.
	\end{equation*}
\end{proposition}
\begin{proof}
Since~\eqref{majorhi} is valid, it follows that, for $x \in A$, we have:
\begin{equation*}
   d_{A\cap C_i} (x) = d_{C_i} (x) \leq \overline{E}\left[ \max_{1\leq i\leq r} h_i(x) \right]^\alpha\text.
\end{equation*}
Moreover, since the condition~\eqref{eq:condredb} holds and the sets $A\cap C_i$ are all bounded, all the hypothesis from the Proposition~\ref{prop:relationdist} are satisfied. Therefore, we have
\begin{equation*}
   d_C( x ) = d_{A \cap C}( x ) \leq M \left[\max_{1\leq i \leq r} h_i( x )\right]^\alpha\text,\quad \forall x\in A\backslash C\text,
\end{equation*}
where $M = \frac{2\left( \frac{D-\rho}{\rho} \right)^{r + 1} - \left( \frac{D-\rho}{\rho} \right)^r - \left( \frac{D-\rho}{\rho} \right)}{\left( \frac{D-\rho}{\rho} \right)-1}\overline{M}$.
\end{proof}

Now, let us notice that if we suppose that the sequence $\{x_k\}$ is bounded, we can assure from Property~\ref{prop:propoptbound} that $\{ x_{k + 1/3} \}$ and $\{ x_{k + 2/3} \}$ are also bounded sequences. Consequently, $\{ \proj_{C_i}( x_{k+2/3} ) \}$ is bounded for all $i=1,\dots, r$ and $\{ \mathcal E^p( x_{k+2/3} ) \}$ should also be bounded if only $\|\mathcal E( x ) - y\| \leq \| x - y \|$ for every $x$ and some $y$, which we assume to be true. Therefore, there exists a compact and convex set $A$ which contains the sequences $\{ x_{k + 2/3} \}$, $\{ \proj_{C_i}( x_{k+2/3} ) \}$, $i = 1, \dots, r$ and $\{ \mathcal E^p( x_{k+2/3} ) \}$, $p \in \{ 1, \dots \}$. Thus, using also Proposition~\ref{prop:intdist}, the argumentation in this paragraph leads to the following:
\begin{corollary}
   Let $C = \bigcap_{i = 1}^r C_i$, where the $C_i$ are closed convex sets. Assume $\inte C \neq \emptyset$, $\{ x_k \}$ is bounded and suppose that $\|\mathcal E( x ) - y\| \leq \| x - y \|$ for every $x \notin C$ and $y \notin C$ and that $\lim_{p \to \infty}d_C\bigl( \mathcal E^p( x ) \bigr) = 0$. Then, if we have $d_{C_i}( x ) \leq M h_i^\alpha( x )$, the scheme defined by~\eqref{eq:repfeaop} with $\phi = \max_{1 \leq i \leq r} h_i$ satisfies Property~\ref{prop:propfac}.
\end{corollary}

That is, given some convergent Féjer-monotone (with relation to $C$) operator $\mathcal E$, in order to obtain a appropriate feasibility operator it is enough to repeat the application of this operator until $\max_{1 \leq i \leq r} h_i$ reaches a small enough value, which is easy to test. We notice that one may tune the stopping criterion in order to minimize the repetition of the operator or to enforce iterates to be nearer to feasibility by choosing large or small values for the constant $K$ in~\eqref{eq:repfeaoptest}, but the influence of this choice in the performance of the algorithm is still an open question.

As for the construction of operators $\mathcal E$, we refer the reader to~\cite[Subsection~3.2]{hed09}, where this matter has been addressed. Without going into details, sequential or parallel application of Polyak-type iterations are sufficient, projections being a special case. More precisely, let, for $\nu \in ( 0, 2 )$ and $\tilde\nabla h( x ) \in \partial h( x )$
\begin{equation*}
   \mathcal S_{h}( x ) := \begin{cases}\displaystyle
                              x - \nu\frac{[ h( x ) ]_+}{ \| \tilde\nabla h( x ) \|^2 }\tilde\nabla h( x ) & \text{if}\ \tilde\nabla h( x ) \neq 0\\
                              x & \text{otherwise}\text.
                          \end{cases}
\end{equation*}
Then, for the case $C = \bigcap_{i = 1, \dots, r}\lev_0( h_i )$, both $\mathcal E_1:= \mathcal S_{h_r} \circ \mathcal S_{h_{r - 1}} \circ \mathcal S_{h_1}$ and $\mathcal E_2 = \frac1r \sum_{i = 1}^r \mathcal S_{h_i}$ are acceptable within our algorithm. As already mentioned \emph{en passant}, by letting $h_i( x ) = d_{C_i}( x )$ and $\nu = 1$, we have sequential (i.e., \textsc{pocs}) or averaged (Cimmino) projections.


\endinput


==> sl_noisy_iter_ssim.tex <==
\def\xaxisLabels{[]\tiny$0$;\tiny$100$;\tiny$200$;\tiny$300$;\tiny$400$[]}
\def\xaxisValues{[]0.00000;0.25000;0.50000;0.75000;1.00000[]}
\def\yaxisLabels{[]\tiny$0.01$;\tiny$0.27$;\tiny$0.54$[]}
\def\yaxisValues{[]0.00000;0.50000;1.00000[]}

